DFL: High-Performance Blockchain-Based Federated Learning

Many researchers have proposed replacing the aggregation server in federated learning with a blockchain system to improve privacy, robustness, and scalability. In this approach, clients would upload their updated models to the blockchain ledger and use a smart contract to perform model averaging. However, the significant delay and limited computational capabilities of blockchain systems make it inefficient to support machine learning applications on the blockchain. In this paper, we propose a new public blockchain architecture called DFL, which is specially optimized for distributed federated machine learning. Our architecture inherits the merits of traditional blockchain systems while achieving low latency and low resource consumption by waiving global consensus. To evaluate the performance and robustness of our architecture, we implemented a prototype and tested it on a physical four-node network, and also developed a simulator to simulate larger networks and more complex situations. Our experiments show that the DFL architecture can reach over 90\% accuracy for non-I.I.D. datasets, even in the presence of model poisoning attacks, while ensuring that the blockchain part consumes less than 5\% of hardware resources.

==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/DFL.tex <==
\section{Technical description of DFL}
\label{DFL_framework}

% \subsection{DFL workflow overview}

Figure \ref{DFL_overview} shows a high-level overview of the DFL workflow. The workflow consists of two event-driven phases. The left phase is triggered when the node has collected enough "ML training data" for training (e.g. when the training data size becomes equal to/larger than the ML batch size). The node will create a "transaction" that includes the new "ML model", and broadcast it to other nodes. After several rounds of communications, the node can generate the "blockchain (proof of contribution)". The right phase is triggered when the node has received enough transactions (controlled by "model buffer" size) from other nodes to update the ML model and ends by updating the "(new) ML model" and "reputation system". 

The blockchain data serves as proof of contribution and can be submitted to a dedicated reward calculation system to quantify the contributions to ML models and distribute the rewards to the DFL nodes. This could be an incentive mechanism to encourage each DFL node to train and share their models.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{image/DFL_Overview.drawio.png}
    \caption{DFL overview}
    \label{DFL_overview}
\end{figure*}

\subsection{DFL workflow}
\label{DFL_workflow}

In this section, a fully-connected four-node DFL system will be used as an example to explain the workflows and structures. Please keep in mind that DFL does not rely on a fully-connected network to operate, less p2p connections also ensure the system's correctness.

Table \ref{notion_table} lists some important concepts which will be used in this section. In the table, either one of the mainstream asymmetric encryption methods, such as ECDSA and RSA, could be applied in the system.

\begin{table*}
    \centering
    \caption{Notion table for Section \ref{DFL_workflow}}
    \label{notion_table}
    \begin{tabularx}{\textwidth}{l|X}
    \toprule
    Notion & Definition\\
    \midrule
    $pri\_key_{node}$ & The private key for a node.\\
    $pub\_key_{node}$ & The public key for a node.\\
    $address_{node}$ & An unique identifier for a node.\\
    $hash(content)$ & The hash for certain content. The content will be immutable once $hash$ is calculated.\\
    $signature(pri\_key, hash)$ & The signature generated by the $pri\_key$ and $hash$.\\
    \midrule
    $generator$ & The node of generating transactions and blocks.\\
    $neighbors\ of\ x$ & All nodes whose network distance to node x is 1.\\
    $further\ neighbors\ of\ x$ & All nodes whose network distance to node x is larger than 1.\\
    \midrule
    \end{tabularx}
\end{table*}


\subsubsection{Node setup}

Each node in the DFL network generates a pair of public/private keys and an address to join the DFL network. The key pair can be generated by most cryptology methods, while the address is produced according to the rule $address_{node} = hash(pub\_key_{node})$.

\subsubsection{Generating transaction and receipt}

Figure \ref{transaction generation} describes the procedures to generate transactions.

\begin{figure*}
    \centering
    \includegraphics[width=0.5\textwidth]{image/transaction.pdf}
    \caption{Procedures of generating transaction and receipt }
    \label{transaction generation}
\end{figure*}

Suppose in our DFL system, node 1 is training at the beginning. The model weights after training are sent to the neighbors of node 1, i.e. nodes 2, 3, and 4 since the network is fully connected. Once other nodes receive the weights, they will start to measure the model accuracy based on their own collected dataset. Each receiver will generate a receipt describing the accuracy of the model, which is then appended at the end of the transaction. The transaction, together with the receipt, will be sent from each receiver to all its neighbors. For instance, node 2 as receiver of model weights from node 1, will send the transaction and receipt to, not only node 1 but also nodes 3 and 4 as well. However, nodes 3 and 4 will ignore the transaction and receipt from node 2, as this transaction has been processed beforehand. Node 1 will collect the receipt for generating the block afterward. 


\subsubsection{Generate block}

Figure \ref{generate block} describes the procedures to generate blocks. Node 1 will gather a certain amount of transactions and corresponding receipts after a certain time. A block would be generated to record the transactions and receipts in order to make them immutable.
\begin{figure*}
    \centering
    \includegraphics[width=0.5\textwidth]{image/generate_block.pdf}
    \caption{Procedures of generating a block}
    \label{generate block}
\end{figure*}

The procedure for generating such a block can be divided into two phases. The block generator creates a draft block in the first phase. The second phase is to gather confirmations from neighbors of the block generator and  finalize a block. With confirmations appended to the final block, the block generator cannot easily modify the previous block as it cannot fake a confirmation.

% confused about these two paragraphs
% Here is one point that transactions will be forwarded but draft blocks will not, because it is most likely for the generator to receive the receipts from its neighbors. The neighbors also will not forward receipts from further neighbors to the generator because the transactions will be treated as duplicates.

Retake the four-node system as an example. Node 1 sends a draft block to node 2, then node 2 will look through the receipts to figure out whether some receipts are produced by node 2 and generate confirmations if there are any. Node 1 will gather all confirmations from nodes 2, 3, and 4 and append the confirmations to finalize the block. The digest of the final block will then be used to generate the next block.

The component diagram is available in Figure \ref{generate_transaction_block_diagram} and Figure \ref{generate_block_block_diagram}. The number before each step indicates the order. These steps present the same process flow as Figure \ref{transaction generation} and Figure \ref{generate block}, so they will not be discussed again.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{image/generate_transaction_struc.pdf}
    \caption{Generating transaction (block diagram)}
    \label{generate_transaction_block_diagram}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{image/generate_block_struc.pdf}
    \caption{Generating block (block diagram)}
    \label{generate_block_block_diagram}
\end{figure}

\subsection{DFL blockchain data format (UML available in Figure \ref{uml:dfl})}
\label{DFL_blockchain_data_format}

In this section, the data formats in the blockchain system will be discussed based on the workflow in previous sections. To be specific, the data formats include the format of the transaction, the transaction receipt, the block, and the block confirmation. These data formats will be used to prove the robustness of the DFL blockchain system.

These data formats will be illustrated in Table \ref{blockchain_notion_table} with some special notions.


\begin{table*}
    \caption{Notion table for Section \ref{DFL_blockchain_data_format}}
    \label{blockchain_notion_table}
    \centering
    \begin{tabularx}{\textwidth}{X|X}
    \toprule
    Notion & Definition\\
    \midrule
    $=\ (operation)$ & This data is obtained by performing the operation.\\
    $hash\ (content)$ & The hash for a certain content, the content will be immutable once $hash$ is calculated.\\
    $signature\ (pri\_key, hash)$ & The signature generated by the $pri\_key$ and $hash$.\\
    $digest\ protected\ (digest\ d)$ & This data is protected by the digest d. If the original data is modified, the digest verification will fail.\\
    \textit{signature protected (signature s, node o)} & This data is definitely generated by $node\ o$ and has not been modified once the signature verification passes. Because a signature is generated based on a digest, all signatures-protected data is also digest-protected.\\
    \midrule

    \end{tabularx}
    % \caption{Blockchain notion table}
    % \label{blockchain_notion_table}
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{image/uml_dfl.drawio.pdf}
    \caption{UML graph for DFL blockchain system}
    \label{uml:dfl}
\end{figure}

\subsubsection{Node information}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{image/uml_node_information.pdf}
%     \caption{UML graph for NodeInformation}
%     \label{uml:node_information}
% \end{figure}

The name of a node is its address. Since the node address is decoupled from the network address, it is hard to access a specific node by its name. This property could achieve similar anonymity as the blockchain since nodes can only receive a trusted transaction from the node but hard to access the generator. For neighbors, they can know each other's network address because they will receive a transaction with no receipt.


\subsubsection{Transaction format}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{image/uml_transaction.pdf}
%     \caption{UML graph for Transaction}
%     \label{uml:transaction}
% \end{figure}

Among all the transaction fields, the $generator$, $create\_time$, $expire\_time$, $ml\_model$, and $ttl$ are protected by the signature, which can only be modified by the transaction creator. A modified transaction with a changed digest will be treated as a new transaction.

The $ttl$ (time to live) is an integer value decreased by 1 when the transaction is forwarded by a node. The transaction will cease being forwarded if its $ttl$ reaches zero. The $ttl$ value is critical for the range of partial consensus. Larger $ttl$ results in a wider partial consensus range with more nodes involved in the accuracy testing for this transaction. So an infinite $ttl$ should be avoided because it might consume too much computing resource. The mechanism to punish a node generating large-$ttl$ transactions can be achieved in the reputation system.

The $expire\_time$ is designed to avoid a late arrived transaction, whose ML model has already been outdated, i.e. processed by other nodes. Those outdated ML models can harm the overall training process and reduce the creator's reputation. This expiration time can as well avoid attackers' attempts to decrease the reputation of the victims by delaying their transactions.

\subsubsection{Receipt format}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{image/uml_receipt.pdf}
%     \caption{UML graph for Receipt}
%     \label{uml:receipt}
% \end{figure}

The $creator$ is the receipt creator, corresponding to nodes 2,3, and 4 in the four nodes example in Figure \ref{transaction generation}. The $transaction\_digest$ is the digest of the received transaction. The transaction digest will not change after appending new receipts because the transaction digest does not take $receipts$ into the computation. The $received\_at\_ttl$ is calculated by the following equation.

\begin{equation}
    \begin{aligned}
    received\_at\_ttl = min(trans.ttl, trans.receipts.received\_at\_ttl) - 1
    \end{aligned}
\end{equation}

The $accuracy$ is tested based on the receipt creator's dataset. In DFL, all nodes will not shuffle their dataset, so a model can have different accuracy for different nodes, especially for non-I.I.D. dataset. The accuracy will be forwarded back to the transaction creator and other nodes. This accuracy information might be helpful for other nodes because it assists to judge the receipt creator's reputation, but it has not yet been implemented in the current DFL version.

\subsubsection{Block format}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{image/uml_block.pdf}
%     \caption{UML graph for Block}
%     \label{uml:block}
% \end{figure}

The $transactions$ in the block are the final collected transactions which contain receipts. Neighbors should verify the correctness of the receipts and generate a block confirmation after verification. The block generator should collect a certain number of confirmations from other nodes in the network in order to finalize the block.
The $genesis\_digest$ is the digest of the genesis block, which records the ML network structure to ensure all nodes use the same ML network. So all nodes in DFL should have the same $genesis\_digest$ if they are training the same model.
The $final\_digest$ is calculated after the block generator collects enough confirmations for each transaction, and will be chained to the next block.

% \subsubsection{Block confirmation format}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{image/uml_block_confirmation.pdf}
%     \caption{UML graph for BlockConfirmation}
%     \label{uml:block_confirmation}
% \end{figure}

% The block confirmation contains $transaction\_digest$, $receipt\_digest$ and $block\_digest$ to prove the block integrity, and the three data segments are signature protected.

\subsection{DFL blockchain properties}

\subsubsection{Asynchronous}
% All nodes are able to work asynchronously because of the absence of global consensus. The generating transaction, block, receipt and confirmation processes on different nodes are independent of each other. The ML process and generating blockchain process are also asynchronous from each other if it is not important to record the contribution in the current block or in the next block.
One of the key features of DFL is its ability to operate asynchronously, as it does not rely on global consensus. This means that the generating transaction, block, receipt, and confirmation processes on different nodes can be performed independently of each other. Additionally, the ML process and the generating blockchain process can also be asynchronous, as long as it is not necessary to record the contribution in the current or next block. This asynchronous nature of DFL allows nodes to operate independently, which can enhance the scalability and efficiency of the system.

\subsubsection{Anonymity}
% All nodes are anonymous on the network, their IP addresses are hidden behind their node addresses and their data packets will only be available to their direct peers. However, the node address might be an identifier for an attacker who wants to recover the dataset held by victims. There are already many blockchain projects such as Monero\cite{monero} to enhance node anonymity, so this paper will not discuss anonymizing node addresses.
All nodes are anonymous on the DFL network, as their IP addresses are hidden behind their node addresses and their data packets are only available to their direct peers. While this anonymity provides some level of protection for nodes, it is important to note that the node address itself may serve as an identifier for an attacker who wants to recover the dataset held by a victim. There are already several blockchain projects, such as Monero \cite{monero}, that aim to enhance node anonymity. However, this paper will not further discuss the issue of anonymizing node addresses.

\subsubsection{Immutability}
% For block generators, a single block will become immutable once it is finalized, because neighbors will not generate block confirmations for a receipt twice. The block generator cannot modify any content in the receipts or confirmation because they are protected by the signature of other nodes. The immutability ensures the contribution to ML models is not modified, and the reward contribution is fair for all nodes.
In DFL, blocks become immutable once they are finalized. This is because neighbors will not generate block confirmations for a receipt more than once, and the block generator cannot modify any content in the receipts or confirmations, as they are protected by the signatures of other nodes. The immutability of blocks in DFL helps to ensure that the contribution to the ML models cannot be modified. This is important for maintaining the integrity of the system and ensuring that all nodes are properly incentivized for their participation.



\subsection{Discussion}
Here are some discussions and comments about the DFL system:

\begin{itemize}
    \item The DFL blockchain data can be deleted to save storage after the contributors have received their rewards. Suppose the reward system for DFL is a smart contract on a traditional blockchain. It is important to minimize the amount of data that is stored on the traditional blockchain, so we should keep the on-chain data minimized to reward algorithm arguments, such as model accuracies. 
    \item In DFL, the communication cost depends on the ML model size, $ttl$, and the number of peers. In traditional blockchain-based federated ML, the communication cost depends on the model size (or gradient size) and the communications in the blockchain system. So the practical communication cost is application-specific and difficult to compare.
    \item Server-side attacks are not applicable because there are no centralized servers. Peer-side attacks, such as model poisoning and dataset poisoning, are a potential concern in DFL.
    \item Privacy attacks are harder to perform in DFL than in a federated learning system because the ML models will only be shared with a limited number of nodes in the network. The ML models in the blockchain data can also be deleted before submitting to the rewarding system if the rewarding algorithm does not require the ML models.
    \item As for network failures, failure to broadcast transactions can cause some transactions to be missed, resulting in fewer contributions to the network and fewer blocks. Failure to send draft blocks results in fewer blockchain confirmations. In practical DFL deployment, each node only needs to collect a certain percentage of confirmations in order to finalize a block. Disconnected nodes can catch up with the rest of the network after re-connection by using a model updating mechanism that gives higher weights to more accurate machine learning models.
    \item An attack method to fake contributions is possible in DFL. This attack method can be described as an attacker that steals the model from other legitimate nodes and generates a new transaction that includes the copied model to gain contributions. Verifying the digest of a transaction does not help because the attacker can slightly modify the model weights to get a completely different digest while retaining similar accuracy. There are two potential ways to defend against this attack. One is to use Trusted Execution Environments (TEEs) \cite{blockchain_TEE} on all nodes to protect the model data. The other way is to use homomorphic encryption \cite{cloud_homomorphic_encryption} to encrypt the model, which allows other nodes to use the model without decrypting it.
    
\end{itemize}



==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/acknowledge.tex <==
\section*{Acknowledgment}

We want to thank Xun Gui and Zixuan Xie for their discussions and ideas on blockchain and machine learning. Their deep insights in blockchain and machine learning helped improve this project. We also thank Kewei Du, Xiaoning Shi and Li Xu for reviewing this paper and providing precious feedback. This research was performed with the support of the European Commission, the ECSEL JU project NewControl (grant no. 826653) and the Eureka PENTA project Vivaldy (grant no. PENT191004).

==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/blockchain_and_machine_learning.tex <==
\section{Blockchain and federated machine learning}
\label{blockchain_and_federated_machine_learning}

This section discusses the design principles of the DFL system and the inspiration behind it. Meanwhile, this section also provides a comparison between DFL and traditional federated ML systems on blockchain. The DFL implementation in Section \ref{DFL_framework} includes more detailed considerations and technical information, while this section only provides the key theory to build a high performance ML system on blockchain.

\subsection{Partial consensus}
\label{partial_consensus}

As previously mentioned, most blockchain systems keep a global consensus. This consensus is essential for a ledger system since miners must validate new transactions based on the current state of each account. Assume two transactions take place in a very short time interval, which are then broadcast to two different nodes quite remote in the network. In this situation, miners would only treat the first received transaction as valid, resulting in different accepted transactions for different miners. But in the blockchain system, only one miner can generate a block which only validates one certain transaction. So the global consensus is critical for the ledger system.

In contemporary cloud computing systems and cloud storage systems, the global consensus is achieved by a centralized server.

However, for ML applications, the global consensus would not be necessary for two reasons. First, the arriving order of transactions is not critical as a late arrived transaction can also be used due to the high tolerance of FedAvg. Second, the model weights in transactions are not critical. Two models might have exactly the same accuracy provided the same test dataset, but their model weights do not necessarily have to be the same.

As discussed in Section \ref{intro_blockchain_system}, global consensus is the cause of bifurcation and contemporary blockchain systems increase the block interval to avoid bifurcation. Nonetheless, the DFL system uses partial consensus rather than global consensus to build a high performance blockchain system for federated ML.

Partial consensus indicates that the models stored in a limited range of nodes should be similar to each other. From the view of network distance, the closer the nodes are, the more similar the models should be. In practice, partial consensus means that the models are only broadcast for a limited distance. All nodes having received this model should take the received model into the next FedAvg iteration. Partial consensus could be an efficient choice because each node does not wait for a global block, which means the traditional synchronized blockchain systems become asynchronous systems. 

Few distributed systems apply partial consensus because of the necessity of a global state. However, as mentioned before, a global state is redundant for machine learning systems. The blockchain database hence becomes the proof of behavior to the contribution of the owner to the model. The proof of behavior in the blockchain also implies the need of having a witness to verify the behavior during the block generation process. In DFL, the witness is the set of neighbors in the p2p network. Neighbors can give feedback on the quality of models by providing the model accuracy based on their own dataset.


Partial consensus can also introduce new vulnerabilities, such as the potential for malicious behaviors like model poisoning to go unnoticed in the network. To address these issues, a reputation system will be introduced in the next section.

% However, partial consensus also brings new vulnerabilities because malicious behaviors, such as model poisoning, can easily hide themselves in this network. So a reputation system will be thrown out to deal with them in the next section.

\subsection{Distributed reputation and weighted federated averaging}
\label{reputation}

The global consensus in a traditional blockchain system ensures no malicious node would dominate the next block, unless they take over more than half of the computation power, called a 51\% attack \cite{blockchain_51_attack}. However, partial consensus allows for malicious behavior such as model poisoning where attackers could easily hide themselves in this network, resulting in new vulnerabilities in the system. A reputation system will be introduced as part of the training ML process to deal with this problem.

There are already some existing reputation systems in the federated ML area. For example,  \cite{reputation_incentive_mechanism} proposed using reputation as an incentive mechanism. The reputation system in DFL is responsible for distinguishing the malicious node in partial consensus. A malicious node can be a node frequently broadcasting low accuracy models, or performing a data poisoning attack or a model poisoning attack. The reputation is distributed and different nodes may rate the same node independently. For example, considering a three-node system - the reputation of node C in node A might be different from that stored in node B. 

The reputation can be updated according to any rational machine learning model criterion. In this paper, we mainly consider updating the reputation according to the model accuracy. More specifically, each node will have its own local reputation record of its neighbors and will update the reputation record based on the accuracy for neighbors' models calculated by itself based on its local dataset. Broadcasting models with higher accuracy earns the node higher reputation in the system. The reputation will be stored locally and not shared with other nodes. 

To protect the system, a malicious node should have a lower reputation in the reputation system. Meanwhile, the influence of malicious models should be lowered as well. We propose using the weighted federated averaging method \cite{weighted_fedavg}, a modified version of FedAvg, in this paper. The modified FedAvg mechanism works together with the reputation system to keep the federated ML secured and stable.


In Section \ref{result_and_discussion}, we implement a sample reputation and weighted average system. However, more factors should be considered for a more universal implementation. These factors include but are not limited to the malicious rate (proportion of malicious node), training performance (the accuracy curve), the data distribution (non-I.I.D. dataset). The variances in these factors will lead to quite different implementations of reputation and weighted FedAvg system. 

DFL is designed to be flexible towards the above variations, such as different dataset distribution, malicious rate, network topology. The reputation implementation and new federated averaging algorithm can be dynamically linked to the DFL framework, while basic tests are performed to ensure the correctness of external reputation and weighted federated average implementation.

\subsection{The blockchain database}
\label{the_block_chain_database}

In traditional blockchain systems, the blockchain database stores all verified transactions and all miners need to process the transactions on the blocks. However, in a partial consensus system, there is no such unique blockchain database, otherwise the system will fall back to a global consensus and struggle with bifurcation. 

In DFL, the blockchain database works as a proof of contribution. The generator needs to generate a block recording the contribution in model training. These contributions should be able to be verified by external nodes in the network. The verification results will be appended to the block forming a final block, whose digest will be used to generate the next block.

With this method, the generator cannot modify the blockchain database because there is no chance to get a second verification. The previous block also cannot be modified as each block is chained by the digest. This property corresponds to the immutability of traditional blockchain.

Though blockchain database is a proof of contribution, it is not a measure of contribution. In traditional blockchain systems, miners can get tokens as rewards for their participation in consensus. In a federated ML system, nodes should be able to get rewards if they trained the model based on their own data. However, the reward is not measured by the amount of transactions (models) in the blockchain database. The reward should be the mixture of reputation and blockchain database. The algorithm to calculate reward, based on blockchain data and reputation, is not covered by this paper. 

==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/conclusion_future_work.tex <==
\section{conclusion}
\label{conclusion_future_work}

This paper presents a new asynchronous federated learning system, integrating a specialized blockchain system to generate the proof of contribution on the ML model. Using blockchain as a distributed proof system rather than a distributed ledger system removes the synchronicity requirement to increase performance. Meanwhile the asynchronicity also introduces the partial aggregation of models in training phase. We implement the architecture as DFL, which contains an executable prototype, a simulator to investigate ML behavior and an SDK to implement and test reputation algorithms. In a four node experiment with MNIST and LeNet, the training accuracy can be up to 90\% while the blockchain overhead can be kept limited to within only 5\% of total execution time. The simulation results show reasonable training accuracy under both non-I.I.D. datasets as well as malicious dataset attacks. However, the reputation mechanism only works in certain model attack cases and requires further research.

% In this paper, we proposed a new blockchain architecture that enables high performance federated machine learning. We implemented the architecture as DFL, which contains an executable prototype and a simulator. In a four node experiment with MNIST and LeNet, the training accuracy can be up to 90\% while the blockchain overhead can be kept limited to within only 5\% of total execution time. The simulation result also shows reasonable training accuracy under both non-I.I.D. datasets as well as malicious node attacks.

% For the machine learning research area, DFL reveals a path to create a decentralized machine learning system with nearly infinite GPU resources which are used to mine cryptocurrency before, once providing proper rewards to participants. For the blockchain research area, DFL establishes a framework for machine learning applications on public blockchain systems, with better privacy, anonymity and performance.

% contribution and numbers
% contribution: 
% numbers: accuracy in conclusion
% For future research purpose, we open sourced the DFL framework at \href{https://github.com/twoentartian/DFL}{https://github.com/twoentartian/DFL}.

% Experiments and simulations show that the DFL system can 很成功的完成训练 and at the same time perform certain robustness with suitable reputation strategy. Key ideas behind the DFL system has potentiality to become a widely used infrastructure in computer science.

% \section{Future work}
% For future research purpose, we open sourced the DFL framework at \href{https://github.com/twoentartian/DFL}{https://github.com/twoentartian/DFL}.

% Here is a summary of possible future work.

% \begin{itemize}

% \item The relationships between data distribution, malicious ratio and reputation, weighted FedAvg implementation requires further research.

% \item Trusted execution environments and homomorphic encryption might be the solutions to model duplication attack. But there are indeed more methods to deal with it. 

% \item Malicious nodes can connect together and fake reputations for each other to attack the network. Though network topology simulation has already been implemented in DFL, we have not yet simulate this attack model.
  
% \item Contribution. The DFL does not implement any mechanism to measure the ML training contribution. Even though the contribution could be derived from the reputation and blockchain database, the reputation of a certain node is distributed among the network where a decentralized and trusted aggregation mechanism is missing. 

% \end{itemize}

==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/high_level_overview_of_dfl.tex <==
\section{High-level overview of DFL}
\label{high_level_overview_of_dfl}

% \textcolor{brown}{Section \ref{high_level_overview_of_dfl} is a new section. Its content is re-arranged from previous Sections 3.1, 3.2, 4.4, 4.5}

% \textcolor{brown}{The presentation of the weighted-federated average is shortened to 2 sentences (in Distributed reputation section) because it is not an inborn feature of DFL.}

DFL is a peer-to-peer (p2p) network where users collaborate for model training by exchanging model parameters. The models are updated asynchronously through i) training when sufficient local data become available to the nodes and ii) averaging when a given number of models are received. DFL applies a local ledger to register the training contribution of each node to be used as an incentive mechanism. DFL implements partial consensus which is more effective in this case, because partial consensus allows each node to do model averaging when they receive models rather than waiting for a block to be finalized. DFL introduces a distributed reputation system to mitigate dataset and model attacks as partial consensus makes attackers hiding easier compared with traditional blockchain-based FL solutions. 

Section \ref{partial_consensus} talks about the partial consensus and its prototype - gossip algorithm in ML. Section \ref{reputation} elaborates on the distributed reputation system. Section \ref{possible_applications} and Section \ref{comparision_of_dfl} show the potential applications of DFL and compare DFL with existing related projects.

\subsection{Gossip algorithm and partial consensus}
\label{partial_consensus}

% \textcolor{brown}{I added the Gossip algorithm here because Reviewer 2 (2nd round) mentioned it and I think it's highly related to the partial consensus}

% As previously mentioned in Section \ref{intro_blockchain_system}, most blockchain systems keep a global consensus. This consensus is essential for a ledger system since miners must validate new transactions based on the current state of each account. Assume two transactions take place in a very short time interval, which is then broadcast to two different nodes quite remote in the network. In this situation, miners would only treat the first received transaction as valid, resulting in different accepted transactions for different miners. But in the blockchain system, only one miner can generate a block that only validates one certain transaction. So the global consensus is critical for the ledger system.

% In contemporary cloud computing systems and cloud storage systems, the global consensus is achieved by a centralized server. However, for ML applications, the global consensus would not be necessary for two reasons. First, the arriving order of transactions is not critical as a late arrived transaction can also be used due to the high tolerance of FedAvg. Second, the model weights in transactions are not critical. Two models might have the same accuracy provided by the same test dataset, but their model weights do not necessarily have to be the same.

% Previous decentralized federated learning research focuses on using gossip algorithms to share models in p2p networks, such as \cite{dfl_gossip} \cite{gossip_algorithm} \cite{Braintorrent}. The gossip method contradicts the global consensus mechanism in blockchain systems because messages will not be broadcast to the whole network in the gossip environment. DFL also applies the gossip mechanism, where each node only shares its models with limited neighbors and invites them to witness of its contribution to ML models.
Gossip algorithms have been a popular choice for decentralized federated learning research, as they enable the sharing of models in peer-to-peer (P2P) networks \cite{dfl_gossip} \cite{gossip_algorithm} \cite{Braintorrent}. DFL also utilizes a gossip mechanism, in which each node only shares its models with a limited number of neighbors and invites them to be witnesses of its contribution to the ML models. While gossip algorithms offer a decentralized approach to model sharing, they may not provide the same level of transparency and trust as a blockchain-based system because single node doesn't obtain the information of the whole network. 

% From the blockchain side, the consensus mechanism for DFL is called partial consensus because an ML model can only be broadcast to a limited range, in contrast with the global consensus where each transaction will be broadcast to the whole blockchain network. Partial consensus is suitable for ML applications for two reasons. First, the arriving order of transactions is not critical as a late arrived transaction can also be used in the current averaging round. Second, the model weights in transactions are not critical. Two models might have the same accuracy provided by the same test dataset, but their model weights do not necessarily have to be the same. 
From a blockchain perspective, the gossip mechanism used in DFL is called "partial consensus", as the ML model (transaction) is only broadcast to a limited range of nodes, rather than the entire blockchain network as in global consensus. Partial consensus is suitable for ML applications for two main reasons. Firstly, the order in which transactions arrive is not critical, as a transaction that arrives late can still be used in the current averaging round. Secondly, the model weights contained in the transactions are not critical. Two models with the same accuracy, as determined by the same test dataset, may have different model weights.

% As discussed in Section \ref{intro_blockchain_system}, the global consensus is the cause of bifurcation and contemporary blockchain systems increase the block interval to avoid bifurcation. Partial consensus loosens the strict synchronization requirement and thus makes room for improving the model communication efficiency, and further reducing the training time. The role of blockchain databases also changes due to partial consensus. The blockchain database serves as proof of the contribution to the ML model. Each node generates and keeps its own blockchain database which records the feedback from neighbors, also known as the witness. Partial consensus can also introduce new vulnerabilities, such as the potential for malicious behaviors like model poisoning to go unnoticed in the network. To address these issues, a reputation system will be introduced in the next section.
As mentioned in Section \ref{intro_blockchain_system}, global consensus in blockchain systems can lead to bifurcation, and many contemporary blockchain systems increase the block interval to avoid this issue. In contrast, the partial consensus in DFL relaxes the strict synchronization requirement and thus allows for improved model communication efficiency and reduced training time. The role of blockchain databases also shifts from an information-sharing system to proof of contribution for the ML models.
% (rather than information sharing), as they serve as proof of contribution to the ML model. 
Each node generates and maintains its own blockchain database, which records feedback from its neighbors (i.e., witnesses). However, partial consensus can also introduce new vulnerabilities, such as the potential for malicious behaviors like model poisoning to go unnoticed in the network. To address these concerns, a reputation system will be introduced in the next section to incentivize honest participation and mitigate the risk of malicious behavior.

% Partial consensus indicates that the models stored in a limited range of nodes should be similar to each other. From the view of network distance, the closer the nodes are, the more similar the models should be. In practice, partial consensus means that the models are only broadcast for a limited distance. All nodes having received this model should take the received model into the next FedAvg iteration. Partial consensus could be an efficient choice because each node does not wait for a global block, which means the traditional synchronized blockchain systems become asynchronous systems. 

% Few distributed systems apply partial consensus because of the necessity of a global state. However, as mentioned before, a global state is redundant for ML systems. The blockchain database hence becomes the proof of behavior to the contribution of the owner to the model. The proof of behavior in the blockchain also implies the need of having a witness to verify the behavior during the block generation process. In DFL, the witness is the set of neighbors in the p2p network. Neighbors can give feedback on the quality of models by providing the model accuracy based on their own dataset.


\subsection{Distributed reputation}
\label{reputation}

There are already some existing reputation systems in the federated ML area. For example, \cite{reputation_incentive_mechanism} proposed using reputation as an incentive mechanism. The reputation system in DFL is responsible for distinguishing the malicious node in partial consensus. A malicious node can be a node frequently broadcasting low-accuracy models, or performing a data poisoning attack, or performing a model poisoning attack. The reputation is distributed and different nodes may rate the same node independently. For example, considering a three-node system - the reputation of node C in node A might be different from that stored in node B. 

The reputation can be updated according to any rational ML model criterion. In this paper, we mainly consider updating the reputation according to the model's accuracy. More specifically, each node will have its own local reputation record of its neighbors and will update the reputation record based on the accuracy of neighbors' models calculated by itself based on its local dataset. Broadcasting models with higher accuracy earn the node a higher reputation in the system. The reputation will be stored locally and not shared with other nodes. 

To protect the system, a malicious node should have a lower reputation in the reputation system. Meanwhile, the influence of malicious models should be lowered as well. We propose using the weighted federated averaging method \cite{weighted_fedavg}, a modified version of FedAvg, in this paper. The modified FedAvg mechanism works together with the reputation system to keep the federated ML secured and stable.

% In Section \ref{result_and_discussion}, we implement a sample reputation and weighted average system. However, more factors should be considered for more universal implementation. These factors include but are not limited to the malicious rate (proportion of malicious nodes), training performance (the accuracy curve), and the data distribution (non-I.I.D. dataset). The variances in these factors will lead to quite different implementations of reputation and weighted FedAvg system. 
In Section \ref{result_and_discussion}, we implemented a sample reputation and weighted average system and obtained promising results. However, there are many other factors that can affect the implementation of this system, such as the malicious rate, training performance, and data distribution. In future work, we plan to investigate the impact of these factors on the reputation and weighted FedAvg system and develop more universal implementations that can handle a wide range of variations.

\subsection{Possible applications}
\label{possible_applications}

This subsection talks about potential applications for DFL. These applications are only feasible with proper reputation algorithms and federated averaging algorithms, which are not covered in this paper.

One potential application is replacing current blockchain-based federated ML systems for less training time and lower resource consumption. Meanwhile, the blockchain database can serve as an incentive mechanism and allow further reward distribution, avoiding the miner fee issue in traditional blockchain-based federated ML systems.

Another possible application is allowing independent developers to deploy their ML models without running expensive cloud servers or paying miner fees. For example, they can embed DFL in their apps to collect data and train models. The reward can be replaced with in-app benefits to compensate users for hardware resources.

% DFL also makes building community-driven ML ecosystems possible. In this ecosystem, developers can propose ML models whose training data comes from users and put advertisements to attract miners to train the models together. A smart contract on traditional blockchain systems can be used to receive DFL blockchain data and distribute token rewards to miners. The token can be used for ML inference in the future if the model is adequately trained. People can buy the token from miners to pay the inference fee. Thus, useful and higher-accuracy ML models should have higher values, represented by the token on the traditional blockchain.
DFL also makes it possible to build community-driven ML ecosystems, in which developers can propose ML models that are trained using data contributed by users and advertise them to attract miners to collaborate on the training process. Smart contracts on traditional blockchain systems can be used to receive DFL blockchain data and distribute token rewards to miners as an incentive for their participation. These tokens can then be used for ML inference in the future if the model is adequately trained, and people can buy the tokens from miners to pay the inference fee. As a result, ML models that are more useful and have higher accuracy are expected to have higher token values on the traditional blockchain, reflecting their perceived value in the ecosystem.

\subsection{Comparison}
\label{comparision_of_dfl}
\cite{9441499} summarizes existing blockchain-based federated ML systems and identifies four major issues that are addressed by these systems: (1) single-point failure, (2) poison attack, (3) lack of motivation, and (4) privacy leakage. Table \ref{tab:comparison_with_other_blockchain_based_FML_systems} lists the addressed issues by each system analyzed in \cite{9441499} and makes a comparison with DFL. The reasons for each addressed issue in DFL are listed below:
\begin{itemize}
    
    \item Single point failure: there is no central server or central ML model, so there is no single point of failure.
    
    \item Privacy leakage: the model in each transaction is a mixture of model training from the dataset and model updating with transactions from other nodes. In addition, each transaction will only be broadcast to limited other nodes due to the $ttl$ mechanism. These two features make privacy attacks much harder.
    
    \item Mining fee: the DFL network avoids mining fees by allowing each node to generate its own blockchain data, unlike traditional blockchain-based federated ML systems that rely on blockchain systems and require mining fees for executing smart contracts.
    % \item Mining fee: traditional blockchain-based federated ML systems rely on blockchain systems to aggregate models. Executing smart contracts on these systems usually needs to pay mining fees. The DFL network does not have mining fees because each node generates its own blockchain data.
    
    \item Synchronicity in the blockchain: DFL is an asynchronous system because it does not require global consensus among the nodes in the network. This asynchronicity can reduce the strict synchronization requirements of traditional blockchain systems to allow for faster training of the ML models.
    \item Lack of motivation: the blockchain data on that node proves the node's contribution to ML models. The contribution is quantified as improvements in accuracy measured by neighbors. The final reward should be calculated by an algorithm (not covered in this paper) involving the blockchain data and the reputations of that node.
    
    \item Poison attack: while the design of a reputation algorithm to prevent poison attacks is not covered in this paper, DFL provides an SDK for further research on this topic. As shown in Section \ref{result_and_discussion}, dataset poison attacks are less effective in DFL because most nodes are innocent. Model poison attacks require additional research.
    % \item Poison attack: it is possible to apply the reputation system in DFL to prevent poison attacks. How to design the reputation algorithm is not covered in this paper, but DFL provides an SDK to support further research on reputation algorithms. According to the results shown in Section \ref{result_and_discussion}. Dataset poison attacks cannot dominate the overall network training once most nodes are innocent. Model poison attacks are more complex and require further research.
\end{itemize}

\begin{table*}[h]
\caption{Comparison with other blockchain-based federated ML systems}
\label{tab:comparison_with_other_blockchain_based_FML_systems}
\resizebox{\textwidth}{!}{%

\begin{tabular}{llll}
\hline
System & Addressed issues & Type of blockchain & Consensus mechanism \\ \hline
BlockFL\cite{block_fl} & Single point failure, lack of motivation & Public & PoW \\
FLChain\cite{fl_chain_1} & Single point failure, lack of motivation & Public & – \\
FLChain\cite{fl_chain_2} & Single point failure & Public & PBFT/PoW \\
RFL\cite{reputation_incentive_mechanism} & Poison attack, lack of motivation & Consortium & PBFT \\
DeepChain\cite{deep_chain} & Single point failure, lack of motivation, privacy leakage & Public & Blockwise-BA \\
FedBC\cite{fed_bc} & Single point failure, privacy leakage & – & – \\
BC-FL\cite{bc_fl} & Single point failure, lack of motivation & Public & Pow \\
BlockFLA\cite{block_fla} & Single point failure, poison attack, lack of motivation & Public \& private & PoW \& PBFT \\
Chain FL\cite{chain_fl} & Single point failure & Private & PoA \\
PSFL\cite{psfl} & Poison attack & – & – \\
BFEL\cite{bfel} & Single point failure, poison attack & Public \& consortium & DPoS/PBFT \& PoV \\
Biscotti\cite{biscotti} & Single point failure, poison attack, privacy leakage & Public & PoF \\
VFChain\cite{vf_chain} & Single point failure, poison attack & Public & Algorand \\
BLADE-FL\cite{blade_fl} & Single point failure & Public & PoW \\
BFLC\cite{bflc} & Single point failure, poison attack, lack of motivation & Public & Committee \\
VBFL\cite{vbfl} & Single point failure, poison attack, lack of motivation & Public & PoS \\ \hline
DFL & \begin{tabular}[c]{@{}l@{}}Single point failure, privacy leakage,\\ mining fee, synchronicity in blockchain,\\ lack of motivation (with a proper rewarding algorithm),\\ poison attack (with a proper reputation mechanism)\end{tabular} & Public & Partial consensus \\ \hline
\end{tabular}
}
\end{table*}

% There are some projects which are similar to DFL but not blockchain-based. IPLS \cite{IPLS} is a decentralized federated learning system based on the inter-planetary file system(IPFS). It also uses a segmented gossip method except that DFL discards the model segmentation mechanism. BrainTorrent \cite{Braintorrent} describes a peer-to-peer federated learning system, which is similar to the DFL federated learning part except that a node needs to actively choose peers and collect models while DFL uses a broadcast mechanism.

There are several projects that are similar to DFL but are not based on blockchain technology. For example, IPLS \cite{IPLS} is a decentralized federated learning system that uses the inter-planetary file system (IPFS) for model dissemination. In terms of federated learning, IPLS applies the segmented model to save bandwidth, which is also different from DFL. Another project, BrainTorrent \cite{Braintorrent}, is a peer-to-peer federated learning system that is similar to DFL in terms of the federated learning process. However, BrainTorrent requires nodes to actively choose their peers and collect models, whereas DFL uses a broadcast mechanism for model dissemination. Overall, these projects demonstrate that there are alternative approaches to federated learning that can be implemented without the use of blockchain technology.


==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/introduction.tex <==
\section{Introduction}

In the past ten years, people have witnessed the rise of crypto-currency and the growth of decentralized finance (DeFi). Most current blockchain applications are limited to the financial domain because it is non-sensitive to performance limitations but relies on data security and integrity. \cite{9441499} and \cite{Li2022} show some potential blockchain application areas such as Internet of Things(IoT) and health care. However, only limited practical applications exist in these areas due to the low transaction per second (TPS) and high latency of blockchain systems.

Federated learning is a machine learning (ML) training method where multiple clients send their local model updates to a central server, which will later generate a new global model and broadcast it to clients. Federated learning addresses privacy issues by keeping the training data on clients \cite{stefan2020}, but it raises trust challenges between clients and central servers. For example, clients can send incorrect models to the central server to harm the global model. Servers can also infer the training data on a specific client using the changes in its model, causing privacy leakage \cite{Protection_Against_Reconstruction_and_Its_Applications_in_Private_Federated_Learning} \cite{https://doi.org/10.48550/arxiv.2101.00159}.

To address the above challenges, some researchers suggest utilizing blockchain technology as a replacement for central servers \cite{fl_chain_1} \cite{block_fla} \cite{fl_chain_2}. This is possible because blockchain offers a transparent and honest environment for generating and broadcasting the new global model. Blockchain also offers a reliable record of the models submitted by clients, thus malicious clients can be identified and removed. Mainstream research in federated learning on blockchain uses smart contracts to perform model aggregation, which results in poor performance because generating a block usually costs over 10 seconds~\cite{chain_fl} \cite{baffle}.

This paper proposes a new blockchain architecture turning the blockchain database from a distributed ledger into a distributed proof of contribution to the ML model, where each node can generate its own blocks asynchronously, significantly improving the overall federated learning efficiency. The new architecture also shows reasonable stability and robustness, with a suitable node reputation strategy and weighted FedAvg implementation for non-I.I.D. datasets and model poising attacks.
From the ML perspective, the main contribution of this paper is an asynchronous Gossip-alike ML training method with blockchain that stores proof of contribution to the ML models. We implement this method in the DFL framework, including an executable prototype, a simulator to simulate the ML behavior, and an SDK to design reputation/model updating algorithms. This paper also mentions other algorithms, such as the reputation algorithm and weighted federated averaging algorithm, but they are not the main contributions because they are used to study the characteristics of the DFL framework.

This paper will first discuss current federated ML and blockchain systems in Section \ref{related_work}. Section \ref{high_level_overview_of_dfl} provides a high-level overview of DFL, as well as its application area and its differences with federated ML. The detailed elaboration, including data format, blockchain structure, and federated ML implementation, is presented in Section \ref{DFL_framework}. Section \ref{result_and_discussion} shows the blockchain performance and federated ML performance. The conclusions and future works are presented in Section \ref{conclusion_future_work}.

==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/related_work.tex <==
\section{Related work and background}
\label{related_work}

\subsection{Blockchain system and bifurcation}
\label{intro_blockchain_system}

Blockchain systems were first introduced in bitcoin \cite{bitcoin_paper}, a peer-to-peer, public and immutable ledger system. All transactions in bitcoin are sealed into blocks to achieve immutability. These blocks are then stored in a directed chain where each block contains the digest of the previous block. The directed chain ensures that any changes in a block will result in the change of all following blocks. Additionally, a global consensus algorithm is applied to ensure that only one chain exists through all nodes in this peer-to-peer network. Bitcoin uses proof of work (PoW) to reach the global consensus, where bitcoin miners must "dig" for a random number to make the block digest meet a certain pattern. The difficulty of finding such a random number varies with the computation power in the whole blockchain network - it becomes more difficult to find a qualified random number with more computational power in total. 

% \subsection{Bifurcation and block generation speed}
% \label{Bifurcation and block generation speed}

In a blockchain system, the computation power of the network is measured by the speed of generating blocks, or equivalently, the interval between two adjacent blocks. This interval time is important for the blockchain system as it determines the probabilities of bifurcation. The term bifurcation describes a situation where in a blockchain network, two nodes generate two correct blocks simultaneously. Since each node only accepts the first block received, one of the blocks would be rejected by over half of all miners. All miners will try to generate the next block based on their current received block. In bifurcation, one block is more likely to generate the next block once it is accepted by most miners because more miners mean more computation resources to find the next block. So as time goes by, one chain will be much longer than the other chains and be accepted by all miners, where the global consensus is reached again. The bifurcation can significantly degrade the performance of the blockchain system and should be avoided. One standard solution is increasing the mining difficulty, which leads to a longer block generation interval. Meanwhile, a longer interval also brings higher latency. However, The bifurcation problem exists in blockchain systems no matter the consensus algorithms.

% \textcolor{red}{More discussion about global consensus will be given in Section \ref{partial_consensus}.}

\subsection{Federated machine learning (federated ML)}

Federated ML continues to draw increasing attention from the research community. A typical federated ML system contains a central server and many clients. The central server is responsible for aggregating and updating the models trained by clients, which are then sent back to clients for the next training iterations. This method of aggregating and updating the central model is called FedAvg \cite{fedavg}. Federate ML has advantages in both data privacy since the training data is privately kept to the client, and model training quality achieves high accuracy for I.I.D., non-I.I.D. and unbalanced datasets \cite{fed_ml}.

However, federated ML also brings new vulnerabilities to the system, including data poisoning \cite{federated_ml_data_poison_1} \cite{federated_ml_data_poison_2}, model poisoning \cite{federated_ml_model_poison_1} and privacy attack from the server \cite{federated_ml_server_privacy_attack_1}. Data poisoning and model poisoning aim to provide wrong models to the central server to harm the training process of the global model. Besides, the central server is able to recover the protected dataset stored on the client by applying Generative Adversarial Networks (GANs) \cite{Zaid_fl_attack} \cite{federated_ml_server_privacy_attack_1}.

Even though federated ML decentralizes ML systems from central servers to client devices, the central server must be kept to perform model aggregation and updating. This makes the central server a single point of failure to the entire system. To deal with this single point of failure and potential attacks on privacy, solutions were proposed where the central server can be substituted by a blockchain \cite{block_fl} \cite{chain_fl} \cite{baffle}. 

\subsection{Federated ML on blockchain}

Bitcoin, as the first blockchain system, has limited functionality as it only provides a distributed and immutable ledger. The next-generation blockchain systems, such as Ethereum \cite{wood2014ethereum}, provide smart contracts to allow users to execute specific small applications on the blockchain system. The smart contract is more reliable because its source code is open to the public on the blockchain and all miners will execute it to ensure the integrity of the results. Some researchers hence attempt to integrate federated ML with Ethereum and replace the model aggregating server with smart contracts \cite{chain_fl} \cite{baffle}. However, applying smart contracts on public blockchain systems is expensive due to the miner fee. Federated ML on blockchains would also be slow because every data aggregation and computation will be performed on all nodes. A brief cost analysis is available in \cite{baffle}, where federated ML costs over $10^8$ Ethereum gas - a cost that would be even greater for larger and more complex ML tasks. This is also the reason why \cite{chain_fl} uses a private blockchain system to avoid high costs. In addition to the above problems, the storage also becomes expensive for federated ML because every model from all ML clients will be stored on all blockchain nodes.

Based on the previous discussion, here is a summary of the problems of current ML approaches to blockchain systems.

\begin{itemize}
  \item Low blockchain performance: limited transactions per block and high latency resulting from long block generation interval.
  \item Mining cost: ML applications must afford the miner fee, which is an extra expense for ML applications.
  \item Excessive storage cost: ML models will be stored on all blockchain miner nodes because the models are stored in a transaction, which will be packed into a block. All miners keep the blockchain database so every single model will be stored on each miner's disk.
\end{itemize}

The above three problems hinder the integration of federated ML on the blockchain, even though there are already many theoretical works to improve the performance of federated ML on the blockchain. For example, \cite{1_bit_awarded_federated_distillation} proposes a compression method to reduce network communication during training; \cite{8843900} focuses on privacy issues in industrial IoT applications. However, only a few of them are built on a real blockchain system \cite{chain_fl} \cite{baffle}.

In this paper, we propose a practical framework (DFL) with 1.~a deployable executable, 2.~a simulator to simulate ML performance, and 3.~an SDK to support further research. 



==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/response.tex <==
\newpage

\section{response to reviewer's comments}

I am sorry that I submitted the response to 1st-round reviewers' comments in the Latex source files, so no 2nd-round reviewer read it.

\subsection{2nd round of revision}

\textbf{Regarding the issues in Figure Simulation results for malicious and non-I.I.D. cases}

\textbf{Reviewer: reduce (or split in different figures) the number of plots in figure 13, logically split Section 5.2 into sub-sections, dividing the explanation of the results of the experiments}

\textbf{We have increased the font size for a better reading experience. Regarding the suggestion of splitting the figure, we discussed it together and would rather not split the figures because of the following reasons: (1) the font size is limited by the number of columns. If we reduce the number of columns, the figures would be harder to compare because we want to compare the accuracy and model weight difference (Y axis) (2) the conclusion in the simulation part is to show that DFL is possible to work in these situations and opens more research topics. Considering that our contribution is not reputation/rewarding algorithms, we'd rather not split its discussion into multiple parts. (3) Table 9 is useful for understanding Figure 89 because it shows the location of the subplots and the meanings of each location. }

\subsubsection{Reviewer 1 (2nd revision)}
\textbf{\#\#\# The design of partial consensus is not clear. A figure could be used to present the partial consensus mechanism.}

\texttt{Partial consensus is moved to Section 3.1. Now "Gossip algorithm" is added to the partial consensus section because it is similar to the idea of partial consensus. The gossip algorithm should be easy to understand because there are already many research papers about it. Introducing the Gossip algorithm first should also clarify the partial consensus.}


\textbf{\#\#\# How are the hyperparameters chosen in this work?}

\texttt{we directly use the hyperparameters in Caffe Lenet to avoid ML-side issues, "We use the same hyperparameters as the LeNet example in Caffe"-Section 5 Result and discussion, 1st paragraph.}


\textbf{\#\#\# To improve the quality of this work, the author should reorganize the structure of the paper, especially for Section 3 and Section 4.}

\texttt{Section 3 and Section 4 are reorganized as suggested by Reviewer 2}


\subsubsection{Reviewer 2 (2nd revision)}
\textbf{\#\#\# In fact, this shows up in Section 5, which needs to  separate the experimentation from the simulation part (the latter stripped of blockchain functionality) I think it would have been fruitful to first prove that the decentralised FL scheme works and in follow-up work, introduce the blockchain-based incentive mechanism}

\texttt{The paper first shows the experimentation because only experimentation can show the resources consumption and further prove our initial motivation: DFL has better performance than existing blockchain-based FL systems, just as the title suggests. Another reason is that experimentation only has 2 or 4 nodes, which is simpler than the 10-node simulations.}

\texttt{Regarding this suggestion "first prove that the decentralized FL scheme works and in follow-up work, introduce the blockchain-based incentive mechanism", our initial thinking is "first show DFL is working (a least in small scale networks) and scaling up to larger networks". However, due to deployment issues and code stability issues, we failed to scale to larger networks, so we turned to using simulations. In addition, we know our decentralized FL scheme, unfortunately, cannot work properly in large-scale networks (50 nodes or above), so I'd rather not use the simulator to "prove" our scheme.} 


\textbf{\#\#\# Key insights may be given by the literature on gossip FL and graph neural networks, but they are not mentioned in the paper (see 3d).}

\texttt{Gossip FL literature is added to Section 3.1 and compared with DFL in Section 3.4}

\textbf{\#\#\# however they are missing very relevant works in the areas of "decentralised FL", "gossip FL", and even "assisted learning". For example,
Pappas, Christodoulos, et al. "Ipls: A framework for decentralized federated learning." 2021 IFIP Networking Conference (IFIP Networking). IEEE, 2021.
replaces the server in FL with a decentralised network, offers a concrete implementation, and is asynchronous. The only distinction is that it uses IPFS instead of blockchain. Its Related Work section (Sec 4) is also highly relevant: see for example
Roy, Abhijit Guha, et al. "Braintorrent: A peer-to-peer environment for decentralized federated learning." arXiv preprint arXiv:1905.06731 (2019).
You will find other works with the keywords that I mentioned above. I would recommend adding a paragraph or two in the introduction discussing / comparing with these solutions}

\texttt{These publications are added to Section 3.1, Section 3.4 and the reference list}


\textbf{\#\#\# Why is blockchain needed in FL? (To remove the server, which is a single point of failure and potentially malicious, offer convenience to developers etc). Has it been done and what were the limitations? (has been tried on public blockchains but is costly, ineffective due to the latency, storage hungry etc.. also a comment on gossip learning and other solutions like in 3d) What does this paper propose and why is it better?}

\texttt{Add two paragraphs in Introduction}

\textbf{\#\#\# I would describe the reputation system in section 4 or even better section 3 as it is really part of the proposal.}

\texttt{DFL provides an interface to design various kinds of reputation algorithms and federated average algorithms, so the reputation algorithm in our paper is just an example of the interface and we don't wish to put it in our major contributions.}

\texttt{In addition, I know there are many limitations in our reputation algorithm and I personally believe it will soon be replaced in the future.}

\textbf{\#\#\# Links to Github should be footnote}

\texttt{Fixed}

\textbf{\#\#\# for the Dirichlet distribution, I would write "For the non-IID samples, we sampled a probability distribution over the class labels for each node based on a symmetric Dirichlet prior. In particular, we investigated the cases a=1 and a=0.1 where  a is a concentration parameter of the Dirichlet distribution meaning etc"}

\texttt{Fixed in Section 5.2}

\textbf{\#\#\# I guess the division with the random numbers refers to \newline https://en.wikipedia.org/wiki/Dirichlet\_distribution\#From\_gamma\_distribution, is that correct?}

\texttt{yes it's correct}

\textbf{\#\#\# please clarify eq 7, Is difference a vector or scalar? is N the number of nodes (one model per node) or the models in the buffer? why sum the weights for each layer and not take the vector difference?}

\texttt{The difference is a vector and each element represents the difference of a layer, the N is the number of nodes/models. Summing the weights of a specific layer in $Model_n$ (because a layer may have thousands of weights) results in a value, and we use that value to represent the layer. So a 4-layer network has 4 vector elements in $Model_n$}

\textbf{\#\#\# There are too many subplots in Fig. 13 and they are rendered so small that they cannot be read. In my opinion, this section should be broken in cohesive units (for example, subsections on no malicious, data poisoning, model poisoning attacks). Now the data generation methods, threat model and evaluation metrics are all mixed together.}

\texttt{I increased the font size of the figure and it should be better now. We would rather not split the figures because (1) the current form is easier to compare and (2) there are many cross-figure analyses in the following part and (3) splitting the figures may exceed the page limitation}

\textbf{\#\#\# usage of "extremely"}

\texttt{Fixed}

\textbf{\#\#\# a reputation system will be "thrown out" to deal with them}

\texttt{Fixed}

\textbf{\#\#\# "high/low performance" is generic, better state directly the metric, e.g., "low latency / accuracy"}

\texttt{Fixed}

\textbf{\#\#\# possibilities should be probabilities (for the Dirichlet distribution)}

\texttt{Fixed}

\textbf{\#\#\# one sentence paragraphs should be avoided}

\texttt{Fixed}


\subsubsection{Reviewer 3 (2nd revision)}

\textbf{the new results section sounds quite confusing (in particular the simulation with non i.i.d dataset and malicious user). In my opinion, the authors should organize the results section in order to make it easier to read and understand. I recommend adding a threat model so that the reader can easily understand the strengths and weaknesses of the DFL framework.}

\texttt{I re-organized the paragraphs in simulation section to make it more clear.}

\texttt{There is an explanation about how attacks are performed in simulation section (5.2) paragraph 3: "There are two types of malicious nodes..."}

\texttt{The simulation section is not meant to illustrate the strength or weakness of DFL. The strength of DFL is that it allows asynchronous ML training in a p2p network with distributed blockchain as a proof of contribution. The weakness is that it makes dataset/model attacks easier so we introduce a reputation system. Section 3 (High-Level overview of DFL) presents similar points. }

\textbf{In the new section 4.4, the authors propose some applications of the DFL framework. My main concern about these applications is that all of them rely on the existence of an incentive mechanism even if it is not part of the contributions of the paper. Several issues may arise in the definition of incentive mechanisms. In my opinion, section 4.4. could be defined as a "future work" considering that it does not present any real-world application for the current version of the DFL.}

\texttt{I agree it's not decent to call them "Applications", so I changed the title from "Applications" to "Possible applications" and added a sentence to tell readers these applications are only feasible with proper reputation algorithm and federated average algorithm.}

\textbf{the choice of incentive mechanism is crucial to fill the "lack of motivation" issues. Considering that the motivation behind the use of blockchain technology is mainly due to the proof of contribution, several issues, about the entity (or entities) responsible for the assignment of incentives, arise.}

\texttt{I agree that there are many blank areas in the reputation and rewarding systems, and the solutions to these issues are application-specific (selection of responsible entity). The blockchain database in DFL is just a proof of contribution to ML models (models are shared with other nodes), it doesn't measure how much contribution is made.}

\textbf{reduce (or split in different figures) the number of plots in figure 13, logically split Section 5.2 into sub-sections, dividing the explanation of the results of the experiments}

\texttt{Please refer to the beginning of the response (2nd revision)}


\subsubsection{Reviewer 4 (2nd revision)}

\textbf{Using the accuracy as a means of computing the reputation of a node does not foster appropriate learning in the face of non-i.i.d. settings. Also, it does not allow to discriminate whether the low accuracy is due to the node being malicious, or having insufficient local data during the learning process}

\texttt{I agree that the current accuracy-based reputation/FedAvg algorithms cannot discriminate malicious and non-i.i.d. nodes. However, there are some misunderstandings about nodes with insufficient training data. Nodes that have insufficient local data for training, will generate fewer transactions and generate fewer blocks, thus getting less reward for model contribution. They can still catch up with the main net if they constantly do model averaging (relevant to the observer concept in Fig 11), and do no harm to the global model. }

\texttt{For extreme non-i.i.d. nodes (e.g. nodes that have training data that no other nodes have, or the training data is so rare that no neighbors can confirm the model contribution), their difference from malicious nodes requires further research.}

\textbf{The article is missing an in-depth analysis to validate one fundamental claim: “this architecture achieves extremely high performance with low resources consumption by waiving global consensus”. In my opinion, this claim should represent the main scope of the article and is currently weakly supported. In order to strengthen its validation, the authors should deepen the DFL performance section by either: Performing experiments that evaluate the DFL performance should also be supported by a comparison with a federated process run under different blockchain systems (e.g., time to reach the same accuracy in the scenario, time needed by each node to perform its own operation under different systems)}

\texttt{I added two paragraphs in Section 5.1 (Result and Discussion - DFL performance) to roughly compare DFL with BAFFLE in terms of execution time. The major difficulty in comparison is that most blockchain-based FL projects are based on simulations and seldom of them have deployment results (blockchain-based FL has become popular yet, either). For projects with deployment results, our test methods are also significantly different. e.g. BAFFLE first trains a global ML model and then records the ML procedures on the blockchain, while in DFL the two processes happen simultaneously. The BAFFLE performance is limited by chunk size(a smart contract parameter), which is, however, just an engineering limitation (because the smart contract concept is not originally designed for ML activities).}

\textbf{However, since the scope is to propose an underlying system based on blockchains, the experiments on the DFL performance are rather poor, and the quality of the system is not properly highlighted by a comparison with other existing blockchain-based systems.}

\texttt{I would like to append some comments after the previous response to "The article is missing an in-depth analysis to validate one fundamental claim...". The major reason for "DFL has higher performance than other projects" is that it releases the blockchain restriction, allowing nodes to do ML activities without waiting for a block to be finalized. In the new submission, Section 3 (High-level overview of DFL), the first paragraph, briefly describes it and Section 4 shows the technical details to show its async property. }

\subsection{1st round of revision}

\subsubsection{Reviewer 1 (1st revision)}

Thank you for your suggestions

\textbf{\#\#\# My main concern for the paper is the actual need for blockchain technology. In general, the blockchain enforces a global state among many nodes in a decentralized manner but, in the proposed solution, each node maintains a separate blockchain that records the transactions related to that particular node. Why is immutability needed in this case? More specifically, it is not clear from the text how the receipts from other users are used. According to my understanding, there are 2 types of accuracies: (1) accuracies for the node's model calculated by neighbors, and (2) accuracies for the neighbors' models calculated by the user. The accuracies from (1) cannot be used as reputation because the other nodes may have faked them, so why are they recorded?} 

\texttt{Thank you for your concern. I realized that I didn't explain the role of the DFL blockchain data. The blockchain data is proof of contribution to ML models. Model designer/company/smart contract can distribute rewards based on this proof and reputation (in other words, it is an incentive mechanism). The "Figure 1 DFL overview" in the revision explains this process and the "DFL framework - Applications" section (changelist 3) gives several examples of using the blockchain data as incentive mechanisms.}

\texttt{It's possible that some malicious nodes will give false accuracies (1) to model generators, causing inaccurate reward distribution. We haven't done any research on it but it should not be big trouble because most nodes should be innocent.}

\texttt{Because the blockchain data is a proof stored on the node's machine, it should be immutable, otherwise, a node can easily discard previous information in the blockchain data and causes inaccurate reward distribution.}

\texttt{The first use of receipts is calculating the contribution to the ML model. The accuracy (1) is immutable before generating a block otherwise the node will not get block confirmation. After generating the block, the accuracy (1) is also immutable until the blockchain data is submitted to the rewarding system.}

\texttt{The rewarding system can be a centralized server if the ML model owner is a commercial company. Or a smart contract on a traditional blockchain system if the ML model is driven by the community. The interval of submitting blockchain data can be relatively long (e.g. one month) to reduce the load.}

\texttt{The accuracy (2) is used to update reputation and update models.}


\textbf{\#\#\# What if the selected neighbors have insufficient data for good training? How can the TTL be adapted?}

\texttt{In DFL, we have a special node type called "observer" node, which only receives and averages models from others and never train the model. This role is used to prevent the case that all nodes can have good accuracies if each node uses IID dataset and self-training dominates the model (which means they seldom share their models).}

\texttt{In result section, "5.3 The speed ratio of model training and model updating", there are some simulations about an observer node.}

\texttt{Observer nodes won't contribute to or damage the global training process, nor generate blockchain to prove his contribution.}

\texttt{TTL is not related to observers here. The TTL is designed to do trade-off between "model broadcast speed" and "network consumption". Larger TTL can let the models broadcast faster but causes larger network flood. }

\textbf{\#\#\# What if the neighbors do not reply, e.g., because of network failures?}

\texttt{There are three cases:}

\texttt{ - Node A fails to send model to Node B: Node A will remove Node B from peer list. This case won't affect the blockchain data.}

\texttt{- Node A sends model to Node B but doesn't get a receipt: The receipts from Node B will be missing in the blockchain file of Node A. But it doesn't matter for Node A because there are other neighbors to proivde receipts.}

\texttt{- Node A sends model to Node B and receives receipt, but fails to send block to Node B or doesn't receive block confirmation. Node A is allowed to finalize the block once he collects enough block confirmations (for example, 80\% of receipts are confirmed). So network failure on a few peers won't bother the blockchain process.}

\textbf{\#\#\# How do the users coordinate to start a training task?}

\texttt{This is a very good question. The answer might sound counterintuitive.}

\texttt{The answer is: coordinations among nodes will slow down the training process (the accuracy grows up much slower). Coordination includes: nodes start training with the same dataset; nodes start training at the same time (and all nodes have the default random model).}

\texttt{There is a special phenomena behind DFL (also applies to all ML systems if they use a similar partial aggregation) and it's not obvious for small size network. For DFL network with over 50 nodes, the phenomena will dominate the training curve. This is also one of the reasons that we don't hope to mention large DFL network because there are too many things to discuss.}

\texttt{If you are interested, you can find the phenomena here\footnote{https://github.com/twoentartian/DFL/blob/main/readme/2021-09-29\%2015:05:15\%20GMT\%2050\%20nodes\%2C\%206peer\%2C\%202\%20observer/accuracy.png}}

\texttt{We will not add the this topic in this paper because it relates to some unpublished work.}

\textbf{}{\#\#\# A comment on the communication cost would be appreciated. For example, could the neighbors return receipts directly instead of flooding to save on bandwidth?}

\texttt{It is hard to make comments on the communication cost due to following reasons:}

\texttt{- In traditional FL, we can send gradients to reduce the communication cost. But in DFL, you must send the whole model. (DFL integrates a compression tool to compress the model and evaluate the performance. This paper doesn't mention it.)}

\texttt{- The communication cost depends on the size of ML model, TTL and the number of peers.}

\texttt{The neighbor send the receipts to other nodes because we want to provide an interface for reputation algorithm to utilize the accuracy from other nodes. The accuracy from other high-reputation nodes might be useful.}

\texttt{Of course, DFL is just a prototype, future projects can remove/add components based on DFL. So we choose to keep flooding for a better reputation interface.}

\textbf{\#\#\# Do the nodes perform training for an epoch and then wait for the models of the neighbors or do they keep training? How does that affect the performance if the nodes do not receive replies?}

\texttt{The new "result" section gives detailed explanations on how training and updating models works.}

\texttt{The node will collect enough data (e.g. data size == batch size) and perform training, after training the node will seal the model in a transaction and broadcast the transaction to other nodes. The "epoch" concept doesn't apply in the DFL because we will never know the complete dataset.}

\texttt{In experiment, the data is randomly selected from MNIST dataset. In simulation, the data is randomly selected with specified distribution. (the distribution is available in the simulator configuration file)}

\texttt{The node will not wait for other nodes. The node only needs to perform model updating when collects enough transactions. The training phases on different nodes are completely asynchronous. Of course the node also needs to generate receipt/block confirmation for other nodes.}

\texttt{The blockchain data is a proof of contribution. It's not a problem if a node sends a transaction to 10 peers but only receives 9 receipts because 9 accuracy feedbacks are enough to characterize its contribution. So missing replies won't influence the performance, it will only make the blockchain proof less accurate.}

\textbf{\#\#\# Do the nodes they wait for their buffer to get filled to average? Do they transmit a model only after an averaging?}

\texttt{Do the nodes they wait for their buffer to get filled to average - yes}

\texttt{Do they transmit a model only after an averaging - no, they transmit a model after training. Figure  1 clarifies this.}

\textbf{\#\#\# What is the impact of the size of the buffer?}

\texttt{Covered in the new "5 Result" section. "The speed ratio of model training and model updating" subsection.}

\textbf{\#\#\# Regarding the reputation mechanism, a key limitation is that it does not work as-is but needs tweaking. Also, can the reputation be reset? Does it apply only for a specific training session?}

\texttt{The DFL framework provides a SDK for updating reputation and models. In the SDK, you can do anything you want. The major problem for reputation is that the algorithm itself is application-specific (e.g. how many attackers are there, the number of parameters, will the trend of data changes, etc)}

\texttt{Also, can the reputation be reset? \-\- yes, once the algorithm requires.}

\texttt{Does it apply only for a specific training session? \-\-depends how you design the reputation algorithm}

\textbf{\#\#\# The implemented network is too simple for meaningful conclusions about the real-life applicability of the solution: 4 fully connected nodes, which can be reached in 1 hop, hiding the impact of TTL}

\texttt{The 4-node fully-connected network is currently our best effort because the DFL is still at the prototype level. Configuring and running this 4-node network without any bugs is already a not-easy work. }

\texttt{In addition, we know there are some hidden "traps" in large-scale DFL networks.}

\texttt{We performed some simulations on 50/100 nodes DFL network, and we found an interesting phenomenon: 
\footnote{https://github.com/twoentartian/DFL/blob/main/readme/2021-09-29\%2015:05:15\%20GMT\%2050\%20nodes\%2C\%206peer\%2C\%202\%20observer/accuracy.png} }

\texttt{We are currently trying to re-produce this phenomenon in deployment. If everything goes well, a paper will come out to discuss it. After that paper, we will do some research about the impact of TTL (hopefully).}

\textbf{\#\#\# Also, the storage and privacy requirements are mentioned in the Introduction but are not addressed later on. There is no comparison, even ball mark estimates, with literature approaches in terms of throughput, computational and communication load. }

\textbf{\#\#\# \- Merge Sections 3 and 4 since they both refer to the proposed method.}

\texttt{Sorry that I won't merge the two sections for the following reasons:}

\texttt{- From my point of view, Section 3 is a very important section, even more important than Section 4, because it elaborates "how" to design an asynchronous \& high-performance ML system on blockchain.}

\texttt{- The DFL framework in Section 4 includes too many unnecessary considerations and technical details (e.g. flooding the accuracy measured by neighbors to other neighbors). Future researchers might have better mechanisms to generate blocks (e.g. without using two communication rounds in generating a block).}

\texttt{- If I merged Section 3 and 4, readers need to think and summarize what is important and what can be discarded.}

\textbf{\#\#\# There is no comparison with other methods in the experimentation section, which is partly justified because the solution is not directly comparable. Nevertheless, there should be at least an approximate analysis of the throughput, latency, and storage benefits of the proposed method, which was the initial motivation.}

\texttt{I mentioned the storage benefits in "4.5 Considerations and comments".}

\texttt{As for the "throughput" and "latency", in traditional blockchain,  "throughput" is how many transactions we can process per second and the "latency" is how many seconds we need to wait until the transactions appear in the block. I don't think these two concepts exist in DFL because the DFL transactions will not reach all nodes. The "latency" also doesn't make a lot of sense for us because DFL is an asynchronous system. It does not matter whether this node is performing machine learning or block generation.}

\texttt{We investigate the blockchain overhead because less blockchain overhead is always desirable.}

\subsubsection{Reviewer 2 (1st revision)}

Thank you for your suggestions

\textbf{\#\#\# The quality of writing of the manuscript may be definitely improved. The discussion of the methodology is quite confusing. Section 3 is full of go-to-sections and, instead of providing the actual design principles as stated by the authors, it seems to be an informal discussion of what is defined in Section 4. The latter instead, which describes the framework, is too concise and it does not highlight in a clear way how the proposed method differs from traditional blockchains. A good way to address these issues could be to merge the two sections, and provide the right amount of both technical details and informal discussion, to allow the reader to get context and the impact more easily. The formatting of these sections does not help: the figures are quite detached from the context they refer to.}

\textbf{\#\#\# Concerning the contributions to FL, the scope of the article is not stated. FL spans on a wide range of applications, from cross-device to cross-silo, which are much different in terms of functional and non-functional requirements. The authors should clarify what are the contexts in which this methodology can be applied.}

\texttt{In fact, I'd rather not use traditional FL terms or concepts because the FL part in DFL is too different from traditional FL. The absence of a global model and updating with partial aggregation of models make the DFL unique in ML area. I still use "FL" in this paper because many algorithms such as FedAvg can be directly ported to DFL, and these two systems share many ML properties. }

\texttt{As for "cross-device" or "cross-silo", I think DFL can work for both types.}

\texttt{Cross-silo: Section "5 RESULT AND DISCUSSION" simulates a non-IID case where each node only has data samples with 2 specific labels.}

\texttt{Cross-device: I don't think "cross-device" can efficiently describe DFL  because there is no "training round" in DFL. For cases where only small portion of nodes can send models to other nodes, Fig 15 indicates (but not prove) that DFL can work properly with limited model broadcasting.}

\texttt{The DFL blockchain system might not work if all nodes frequently go online/offline in cross-device cases, but the ML side can work properly with a broker to temporarily store and forward the models. }

\textbf{\#\#\# The choice of the update rule for the model aggregation is completely wrong. Evaluation of the received model on a local dataset to measure the accuracy and, consequently, the reputation of another node for weighting the contribution of the model to the update misses the main point of federated learning: learning a global model, or increasing the local performance in the face of lack of data.}

\texttt{I am not sure I understand what's your concern here because, from my point of view, the model aggregation in DFL is completely from FL (Section 3 and Section 4 have already shown the DFL mechanism), and the model update rule in DFL of course will miss the main point of traditional FL.}

\texttt{By the way, I would like to address that there is no "global model" in DFL. }

\textbf{\#\#\# With the use of this aggregation rule, models which work on a different local distribution (which may be the more informative), are penalized by the statistical heterogeneity, instead of taking advantage of it. }

\texttt{Models working on a more informative dataset should have higher accuracies on the other nodes' dataset and take more weight in the other nodes' updating process. The model generator can record these accuracies in blockchain as proof of contribution.}

\textbf{\#\#\# Furthermore, there is no mention about how the evaluation dataset is designed, which brings me to the last point.}

\texttt{The new "result" section explains how test dataset is selected. The test dataset in experiment is randomly selected from all received data samples. The test dataset in simulation is randomly selected from the MNIST test dataset.}

\textbf{\#\#\# The experimental assessment has too many blind spots. There is no mention about how the data was split between nodes, what is the “test set” where the local models are evaluated (is it a local split of the data? An external global dataset?), how many training epochs a node performs before starting the transactions. }

\texttt{Thank you for your suggestion. I re-wrote the whole "result" section, and this version contains a detailed deployment configuration. The configurations for simulation are also open-sourced on Github, and there will be direct links to them.}

\texttt{In the experiment, all nodes get a certain amount of samples randomly selected from the MNIST dataset every second (different data samples for different nodes). Each node performs training once the received data >= batch size and broadcasts the trained model to other nodes. We don't use epochs anymore because nobody knows what's the whole dataset in a p2p network.
In the revision, the new "Section 5 Result" should clarify this point.}

\textbf{\#\#\# Also, the experiment depicted in section 6.5 seems to hide a crucial point of what I mentioned before about the aggregation rule. If the data is i.i.d. across 4 clients, while there is a malicious node, it seems naïve that the other nodes’ models will be ranked higher: their learning process is proceeding on approximately the same distribution, and they will perform well on each of the others’ local datasets. But what happens if the data is non-i.i.d. across clients and the guarantee of the malicious node being ranked lowest comes less? This should be investigated, too.}

\texttt{I hope Section 5.2 and Fig 13 in revision can answer this question. In non-I.I.D. + dataset poisoning cases, the model will be trained slower but still reaches an acceptable accuracy. In non-I.I.D + model poisoning cases, you are correct that there is no guarantee that the malicious node will be ranked lowest. We need more complex reputation algorithms to identify malicious nodes and non-IID nodes. The sample reputation algorithm is only used to prove the DFL framework works, and it's not our major contribution. The major contribution of this paper is solving the performance issue in traditional ML on blockchain systems by asynchronizing the blockchain and ML. }

\textbf{\#\#\# Finally, in table 5, experiments show a huge overhead given by the blockchain system (and by the “calculate accuracy” operation for computing the reputation) even with four nodes. Provided that the FL scenarios are inherently massively parallel, I am very skeptical about both the applicability of the framework and the trade-off between costs and benefits in terms of security. Even if the framework allows for a faster update between local nodes, propagating the nodes’ updates to the whole network may still be really costly.}

\texttt{1. The experiment result is CPU time. 1 second means a CPU core runs for 1 second rather than 1 physical second.}

\texttt{2. The time spent on "Calculate accuracy" and "broadcasting" is proportional to the number of peers. And a single node usually only has limited peers. In the revision, we simulate a 10-node network with each node having 4 peers.}

\texttt{3. The nodes’ updates will never be propagated to the whole network. There is an integer called "TTL" in transactions. TTL will be reduced by 1 once forwarded, and the node will stop broadcasting the transaction if TTL reaches 0. Because TTL can be defined in the genesis block and each node has the same "initial TTL" value, it is impossible for a node to broadcast the transaction to the whole network. In our experiments and simulations, the TTL is fixed to 1.}

\subsubsection{Reviewer 3 (1st revision)}

Thank you for your suggestions

\textbf{\#\#\# the authors should add a presentation of the related works. The "RELATED WORK" section only introduces the topics covered in the manuscript without referring to other solutions proposed to solve the integration of the federated learning algorithm in the blockchain technology;}

\texttt{From our limited knowledge, the most-related and widely-applied solution is to integrate federated ML with blockchain technology using smart contracts to do model aggregation and model updating. I have already mentioned it in Section "2.3 Federated machine learning on blockchain".}

\texttt{There are also many blockchain-level acceleration methods, such as layer-2, and side-chain, but they are unrelated to this paper. Mentioning them here might let readers think we will propose a similar thing. However, DFL is fundamentally different from them.}

\texttt{There is also a lot of research about building/optimizing the federated ML on the blockchain on the theoretical level, but no research addresses the poor blockchain performance. Because the DFL framework focuses on performance, mentioning these researches might mislead readers.}

\texttt{As far as we know, there are only two papers (ref 10, ref 17) deploying ML applications on a practical blockchain project, and both of them are mentioned.}

\texttt{BTW, I changed the section name from "RELATED WORK" to "RELATED WORK AND BACKGROUND"}

\textbf{\#\#\# Section 3.4 introduces the reader to the Weighted federated averaging }

\textbf{\#\#\# although the reference [22] describes the FedAdp algorithm. Which algorithm do you use and why? I suggest adding the reasons that led to the choice of the algorithm used.}

\texttt{In the new result section, we give each algorithm a name: "HalfFedAvg" and "Reputation-0.05".}

\texttt{I don't think other papers will mention similar algorithms because they don't need to keep 50\% old models (the old model contributes 50\% of the new model in updating process). DFL needs the old model because the peers is not trustworthy and only "my own model" is trustworthy.}

\texttt{The major contribution of DFL is not FedAvg algorithms and the algorithms are only used to show the DFL works (we add this point in the new "1. introduction" section).}

\texttt{In addition, I don't think there is too much research value in our FedAvg algorithms. I believe future researcher can design something better. }

\textbf{\#\#\# \- It is not clear how the framework set the configuration of the federated learning algorithm (e.g. federated rounds, local epochs, loss function). Considering the algorithm used to define the reputation, it needs several federated rounds to "identify" a malicious user. For this reason, I think it is important to specify the configuration of the federated learning algorithm and, probably, the related assumptions/limitations.}

\texttt{The "result" section has been completely rewritten. And the new "Result" section should answer most of the configuration questions in our simulation.}

\texttt{The configuration files to reproduce the result is open-sourced and you can find the links in the paper.}

\texttt{I can briefly answer it here: we don't use "federated rounds", "local epochs". "local epochs" is replaced by "how many training samples injected per tick". "federated rounds" doesn't exist because it is a kind of synchronization, and DFL is completely asynchronous. The loss function is the original loss function for LeNet/MNIST (sparse\_categorical\_crossentropy).}

\textbf{\#\#\# the experiments involve only one dataset and one model. I suggest extending the experimental evaluations on different datasets (e.g. federated learning benchmark) and different models. It could be interesting to test the framework using simpler models and add a comparison with the results obtained using a traditional ML configuration algorithm. }

\texttt{Thank you for your suggestion. Our develop team will add support for ML models and dataset in the future. Currently we are doing some work about "large-scale DFL network" and don't have extra time to implement interface for other ML models and datasets.}

\texttt{By the way, the major contribution of DFL is the partial aggregation of models and integrating ML with blockchain in an asynchronous way. Supporting more ML models and dataset does not add extra value to our major contribution point, so we can only do it in the future.}

\textbf{\#\#\# the experiment with the Non-I.I.D dataset should show the distribution of the training example among the nodes. It is only specified that the partitions follow a Dirichlet distribution without showing the actual number of examples per class owned by each node.}

\texttt{We didn't do any experiments with the Non-I.I.D. dataset, I guess you mean simulations.}

\texttt{In the new result section, all simulations configurations are open-sourced. We don't directly put the distribution of the training example on the paper because there are too many. You can find a link to these configurations (in Section 5.2 ML properties (simulation).}

\textbf{\#\#\# it is not clear how the FedAvg buffer works.}

\texttt{We added Fig 1 DFL overview and it mentions how model buffer (FedAvg buffer) works.}

\texttt{The result section also describes the model buffer parameters for simulation and experiments.}

\textbf{\#\#\# the DFL supports only the accuracy metric that, in several machine learning tasks, is not a good indication of the model performances. Is it possible to generalize the proposed approach with other metrics? }

\texttt{Thank you for your suggestion. I think our development team will discuss more ML metrics in the future.}

\texttt{During this revision, we add a metric called "model weight difference", which can describe how different the models in the DFL network are. This metric shows many interesting results that require further research.}

\textbf{\#\#\# the structure of the manuscript presents several sections with a short description. I strongly suggest reviewing the structure and flow of the paper by gathering sections in macro-topic with an in-depth description of the topics presented.}

\texttt{We have reviewed the structure, and many small sections have been merged into a large one. Our modifications are based on the suggestions from the first reviewer because he also mentioned this problem.}

\texttt{BTW, I feel like I didn't clarify what are the major contributions of our paper. So I add a paragraph to explain the major contribution in section "1. Introduction". The section "4.4 Applications" also describes some possible applications to elaborate our contribution.}


==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/result.tex <==
\section{Result and discussion}
\label{result_and_discussion}

This section uses experiments to measure the DFL performance and simulations to investigate the ML properties regarding malicious nodes and non-I.I.D. datasets \footnote{DFL source code available: \href{https://github.com/twoentartian/DFL/tree/9d8d0a2a4e5e05e91460d005a567a8c73b608739}{\texttt{https://github.com/twoentartian/DFL/tree/9d8d0a2a4e5e05e91460d005a567a8c73b608739}}}. 
% There is a manual on the project homepage to let developers compile the DFL simulator and deploy the DFL networks. 
We also upload the simulation configuration files and reputation binary files to make the simulation results re-producible. 
% The experiment results are harder to reproduce because the performance results are subject to the DFL deployment environment and computer performance.
The ML model used in our experiment and simulations is LeNet \cite{LeNet}, and the dataset is MNIST \cite{deng2012mnist}. We use the same hyperparameters as the LeNet example in Caffe \cite{lenet_caffe_hyperparameter} because improving the ML models is not our focus. We implement two types of reputation and weighted FedAvg methods. The first implementation is a slightly modified version of federated averaging without reputation. The following formula describes the model updating procedure on each node:

\begin{equation}
\label{eq:HalfFedAvg}
    model_{next} = \frac{\sum_{n=1}^{N} \frac{1}{N} \cdot model_{n} + model_{prev}}{2}
\end{equation}

The $model_{next}$ is the output model of this model updating iteration, $model_{n}$ represents the received models from other nodes, $model_{prev}$ is the local output model of the last model updating iteration. $N$ represents the total number of models in the model buffer. This formula does not utilize the reputation mechanism, and we call this formula "\texttt{HalfFedAvg}" in this paper because, in this formula, each node's own model contributes to 50 percent of the new model, while models received from other nodes together contribute the other 50 percent.
% We call this mechanism "\texttt{HalfFedAvg}" in this paper because it doesn't utilize reputation mechanism and both external models and own models contribute to 50 percent of the new model.

The second implementation is called "\texttt{reputation-0.05}", as described in the following formula:

\begin{equation}
    weight = reputation \cdot accuracy
\end{equation}

\begin{equation}
\label{eq:Reputation_0.05}
    model_{next} = \frac{\sum_{n=1}^{N} \frac{weight_{n}}{\sum_{m=1}^{N}weight_m} \cdot model_{n} + model_{prev}}{2}
\end{equation}

$reputation$ is the reputation of the model generator, ranging from 0 to 1. The node with the lowest accuracy will be punished by reducing its reputation by 0.05 in each iteration (the punishment will stop if the reputation is already 0). $accuracy$ stands for the calculated accuracy from the model in the transaction, ranging from 0 to 1. Suppose there are $N$ models in the FedAvg buffer, the total weight is obtained by summing all weights (like in the denominator $weight_m$), and the previous model is marked as $model_{prev}$. A special case in "\texttt{reputation-0.05}" is that the reputations of all peers become 0. In this case, the mechanism will be replaced by "\texttt{HalfFedAvg}".

% \begin{equation}
% \label{eq:Reputation_0.05}
%     model_{output} = \frac{\sum_{n=1}^{N} \frac{weight_{n}}{weight_T} \cdot model_{n} + model_{prev}}{2}
% \end{equation}

% $reputation$ is the reputation of the model generator, ranging from 0 to 1. The node with lowest accuracy will be punished by reducing its reputation for 0.05 in each iteration. $accuracy$ stands for the calculated accuracy from the model in the transaction, ranging from 0 to 1. Suppose there are $N$ models in the FedAvg buffer, the total weight ($weight_T$) is obtained by summing all weights, the previous model is marked as $model_{prev}$. A special case in "\texttt{reputation-0.05}" is that the reputations of all peers become 0. In this case, the mechanism will be replaced by "\texttt{HalfFedAvg}".

We note here that the algorithms and mechanisms introduced above are not the main contributions of this paper. The main contribution of this paper is the DFL framework itself, and the above algorithms are used to show the DFL framework is possible to be applied in malicious and non-I.I.D. cases.

\subsection{DFL performance (experiment)}
The goal of this experiment is to investigate the performance of the DFL network. The built-in performance profiler in the DFL executable can measure the CPU time consumed by each task in the DFL components (generate block, generate transactions, update models and receive transactions). The GPU acceleration in Caffe is disabled to ensure the metric of CPU time is fair for ML and blockchain tasks.
We provide two DFL testnets, a four-node net, and a two-node net. Both testnets use the "\texttt{reputation-0.05}" mechanism.

\subsubsection{The two-node net}
The two-node test net is configured as each node will receive eight randomly-selected data samples from the MNIST training dataset per second. The training batch size is 64, so each node will perform a training every 8 seconds in theory. A transaction will be generated and broadcast immediately after the training. Each node will generate a block after broadcasting 4 transactions, equivalent to 32 seconds. The test batch size is 100, and each node will randomly choose 100 samples from all received samples. We do not use the test dataset here because choosing from received samples is closer to practical cases. On a higher level, other DFL nodes with different received samples can replace the role of the test dataset. The FedAvg buffer size is set to 4, causing the FedAvg and reputation mechanism to run roughly every 32 seconds.

Figure \ref{fig:experiment_2_node_accuracy} shows the accuracy graph. The accuracy is tested based on local received data on each node. It causes a rapid increase (from 0s to 30s) in accuracy at the beginning of training. The rapid drop near 32 second is caused by the FedAvg process, which merges the models from other nodes with different datasets. Table \ref{tab:2_node_performance} shows the performance result and Table \ref{tab:2_node_blockchain_statistics} shows the blockchain statistics. The performance result indicates that the blockchain part (blockchain overhead) only consumes a small portion of CPU time, the network (broadcast transaction, gather confirmation and broadcast generated transaction) consumes much more, and ML (calculate accuracy, calculate self-accuracy and measure accuracy) costs the most. In DFL, the blockchain data is proof of contribution to ML models, and spending less time generating such proof is always desirable.

Notice that the time in Table \ref{tab:2_node_performance} is CPU time while the time in Figure \ref{fig:experiment_2_node_accuracy} (x-axis) is wall clock time. Because DFL is a multi-threading application, summing all time in Table \ref{tab:2_node_performance} will result in a larger value than wall clock time.

\begin{figure}[h]
    \centering
     \includegraphics[width=0.5\textwidth]{image/2_exp.pdf}
    \caption{Accuracy graph for 2 nodes}
    \label{fig:experiment_2_node_accuracy}
\end{figure}

\begin{table}[h]
\centering
\caption{Two node performance result, unit: CPU second}

\begin{tabular}{l|cc|ccc}
\hline
\multirow{6}{*}{node-1} & \multicolumn{2}{c|}{Generate block (s)} & \multicolumn{3}{c}{Generate transaction (s)} \\ \cline{2-6} 
 & Gather confirmation & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & Broadcast transaction & Measure accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 21.52 & 3.48 & 59.10 & 362.83 & 18.31 \\ \cline{2-6} 
 & \multicolumn{2}{c|}{Update model (s)} & \multicolumn{3}{c}{Receive transactions (s)} \\ \cline{2-6} 
 & Calculate self-accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & \begin{tabular}[c]{@{}c@{}}Broadcast generated \\ transaction\end{tabular} & Calculate accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 82.94 & 0.94 & 80.57 & 341.73 & 5.50 \\ \hline
\multirow{6}{*}{node-2} & \multicolumn{2}{c|}{Generate block (s)} & \multicolumn{3}{c}{Generate transaction (s)} \\ \cline{2-6} 
 & Gather confirmation & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & Broadcast transaction & Measure accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 22.22 & 2.40 & 72.81 & 312.30 & 7.18 \\ \cline{2-6} 
 & \multicolumn{2}{c|}{Update model (s)} & \multicolumn{3}{c}{Receive transactions (s)} \\ \cline{2-6} 
 & Calculate self-accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & \begin{tabular}[c]{@{}c@{}}Broadcast generated \\ transaction\end{tabular} & Calculate accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 77.16 & 0.43 & 44.89 & 310.63 & 3.62 \\ \hline
\end{tabular}%

\label{tab:2_node_performance}
\end{table}

\begin{table*}[h]
\centering
\caption{Two node blockchain statistics}
% \resizebox{\textwidth}{!}{%

\begin{tabular}{ccccc}
\hline
 & Transaction/Block & Confirmation/Block & Peers & Block \\ \hline
node-1 & 4 & 4 & 1 & 24 \\ \hline
node-2 & 4 & 4 & 1 & 24 \\ \hline
\end{tabular}%

% }
\label{tab:2_node_blockchain_statistics}
\end{table*}

\subsubsection{The four-node net}
Some configuration modifications are applied to the four-node DFL network: the training sample received by each node is decreased from 8 to 4 per second; the FedAvg buffer size is increased from 4 to 8; the transaction count in each block is increased from 4 to 12. The network topology is fully-connect. The results are shown in Figure \ref{fig:experiment_4_node_accuracy}, Table \ref{tab:4_node_performance}, and Table \ref{tab:4_node_blockchain_statistics}.

\begin{figure}[h]
    \centering
     \includegraphics[width=0.5\textwidth]{image/4_exp.pdf}
    \caption{Accuracy graph for 4 nodes}
    \label{fig:experiment_4_node_accuracy}
\end{figure}


\begin{table*}[h]
\centering
\caption{Four node performance result, unit: CPU second}


\begin{tabular}{l|cc|ccc}
\hline
\multirow{6}{*}{node-1} & \multicolumn{2}{c|}{Generate block (s)} & \multicolumn{3}{c}{Generate transaction (s)} \\ \cline{2-6} 
 & Gather confirmation & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & Broadcast transaction & Measure accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 56.63 & 3.17 & 71.72 & 364.72 & 8.28 \\ \cline{2-6} 
 & \multicolumn{2}{c|}{Update model (s)} & \multicolumn{3}{c}{Receive transactions (s)} \\ \cline{2-6} 
 & Calculate self-accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & \begin{tabular}[c]{@{}c@{}}Broadcast generated \\ transaction\end{tabular} & Calculate accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 90.34 & 0.74 & 214.48 & 1944.49 & 23.33 \\ \hline
\multirow{6}{*}{node-2} & \multicolumn{2}{c|}{Generate block (s)} & \multicolumn{3}{c}{Generate transaction (s)} \\ \cline{2-6} 
 & Gather confirmation & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & Broadcast transaction & Measure accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 105.66 & 4.00 & 88.89 & 399.76 & 8.86 \\ \cline{2-6} 
 & \multicolumn{2}{c|}{Update model (s)} & \multicolumn{3}{c}{Receive transactions (s)} \\ \cline{2-6} 
 & Calculate self-accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} & \begin{tabular}[c]{@{}c@{}}Broadcast generated \\ transaction\end{tabular} & Calculate accuracy & \begin{tabular}[c]{@{}c@{}}Blockchain \\ overhead\end{tabular} \\ 
 & 99.67 & 3.45 & 299.28 & 1438.01 & 20.07 \\ \hline
\end{tabular}%

\label{tab:4_node_performance}
\end{table*}

\begin{table}[h]
\centering
\caption{Four node blockchain statistics}
% \resizebox{\textwidth}{!}{%

\begin{tabular}{ccccc}
\hline
 & Transaction/Block & Confirmation/Block & Peers & Block \\ \hline
node-1 & 12 & 35.11 & 3 & 9 \\ \hline
node-2 & 12 & 35.67 & 3 & 9 \\ \hline
\end{tabular}%

% }
\label{tab:4_node_blockchain_statistics}
\end{table}

In theory, the \texttt{Confirmation/Block} value should be 36 because each transaction has 3 confirmations, and there are 12 transactions in a block. The real value is slightly smaller because some confirmations are not collected in time. In practical deployment, the rule of finalizing a block could be "collecting at least 80 percent of all confirmations" or "collecting at least 60 percent of confirmations for each transaction" to make trade-offs on the blockchain robustness and performance.

As shown in Table \ref{tab:4_node_performance}, most CPU resources are consumed by calculating the accuracy of received models, and this time consumption is directly proportional to the number of direct neighbors. Given that the number of neighbors is restricted to a specific maximum and that the workflow on each node is asynchronous from that of other nodes, DFL does not suffer from blockchain-related scalability issues as the number of nodes in the network increases.

To illustrate that DFL has higher performance compared to other blockchain-based FL systems, we compare it to Baffle \cite{baffle}, a federated learning system based on a private Ethereum network with Proof-Of-Authority consensus. The results of this comparison are shown in Table \ref{tab:compare_dfl_baffle}, which indicates that the time consumed by the DFL blockchain part is 10 times smaller than Baffle. It is important to note here that the blockchain performance in Baffle is affected by the "chunk size" parameter (which is not an issue for DFL). Additionally, the reason why we do not use wall-clock time for DFL in Table \ref{tab:compare_dfl_baffle} is that it is determined by the manually-set training data injection rate.


\begin{table}[h]
\centering
\caption{Time comparison: DFL vs Baffel}
\begin{tabular}{|l|l|l|}
\hline
 & DFL & BAFFLE \\ \hline
Model & LeNet & 2-layer DNN, 500 perceptrons each layer \\ \hline
Number of nodes & 2$\sim$4 & 16$\sim$128 \\ \hline
ML-related activities & 2000s$\sim$2500s (CPU time) & 70s$\sim$90s (wallclock time) \\ \hline
Blockchain-related activities & $\sim$200s (CPU time) & \begin{tabular}[c]{@{}l@{}}2000s (chunk size \footnote{chunk size is a blockchain parameter in BAFFLE \cite{baffle}} 16kB) - \\ 11000s (chunk size 2kB) (wallclock time)\end{tabular} \\ \hline
\end{tabular}
\label{tab:compare_dfl_baffle}
\end{table}

Despite the conclusion that the blockchain part only consumes little CPU resources, the result shows another conclusion that the CPU time consumed by calculating accuracy for models from other nodes is proportional to the number of peers. In our experiments, calculating accuracy is a bottleneck for performance because it delays replying to receipts. Re-performing the experiment with GPU accelerators may solve this bottleneck. In real deployments, the number of peers should be controlled to save hardware resources.


\subsection{ML properties (simulation)}
\label{subsection:ml_propertires}
In this section, an investigation is conducted to assess the effect of non-I.I.D. datasets and malicious nodes on machine learning. Due to some limitations in deploying larger DFL networks, we use a simulator to replace the actual deployment.

\begin{itemize}
    \item The DFL simulator removes the blockchain part.
    \item In DFL deployments, each node is asynchronous because they run on different computers. The simulator is a single process, and its behavior is synchronous, so we use a virtual time scale, called "Tick", to simulate the asynchronous behavior. For example, each node receives a batch of training data every "x" ticks, the "x" is a random value between 8 to 12.
    \item The DFL simulator does not simulate delay. The delay includes network delay and the time spent on ML. For example, a node will know the accuracy of a model from other nodes immediately once broadcasted. 
    \item In simulator, the accuracy values are always calculated based on the MNIST test dataset rather than based on the actual received data samples received by each node.
\end{itemize}

We investigate three non-I.I.D. types of dataset. The first type is that each node only gets a dataset with two specific labels. For example, node-0 only gets training data labeled with 0 and 1; node-1 only gets training data labeled with 1 and 2. 
% The other two types of non-I.I.D. assign random numbers to each label with a Dirichlet distribution, representing the possibilities of appearing in the training dataset. 
For the other two types of non-IID samples, we sampled a probability distribution over the class labels for each node based on a symmetric Dirichlet prior. In particular, we investigated the cases \texttt{alpha}=1 and \texttt{alpha}=0.1 where \texttt{alpha} is a concentration parameter of the Dirichlet distribution.
% The possibility is calculated by dividing the random number of a specific label by the sum of random numbers from all labels. The \texttt{alpha} of the Dirichlet distribution represents how non-I.I.D. the dataset would be, 
Smaller \texttt{alpha} results in a more non-I.I.D. dataset. For non-I.I.D. cases described by the Dirichlet distribution, we will regenerate the probabilities of each label and repeat the simulation 10 times to avoid extreme results.

There are two types of malicious nodes: dataset-poisoning attackers and model-poisoning attackers. Dataset attackers always use random samples (all pixels are uniform random numbers from 0 to 1) to train models and send them to other nodes. Model attackers train the model normally but always send randomly generated models to other nodes. The weights of the model are uniform random numbers from 0 to 0.001. We choose 0.001 as the maximum weight value to avoid NaN (floating-number overflow) error in Caffe. The output of the random model is also random because of the last Softmax layer.

The DFL simulation network contains 10 nodes, and each node actively connects to two other peers, so in theory, each node will have 4 peers if no overlapping occurs. The network topology is randomly generated by a DFL tool, and all simulations in this section use the same network topology. The FedAvg buffer size is 4 regardless of peer count. The training batch size is 64, and the test batch size is 100. Each node will get a batch of training data at the training tick, which is determined as the current training tick plus a random number ranging from 8 to 12. The transaction $ttl$ (defined in Figure \ref{uml:dfl}) is fixed to 1. 

The DFL simulator provides two metrics. The first metric is the model accuracy of each node, and the second metric is a value to describe how different the models are. The following formula calculates the value:

\begin{equation}
    \textit{difference} = \frac{\sum_{n=1}^{N-1} {| model_n - model_{n-1} |} + | model_0 - model_n | }{N}
\end{equation}

The $N$ represents the number of nodes \footnote{also represents the number of models because each node has one model}, $model_n$ indicates the sum of the weights for a specific layer of model $n$. $model_n$ is a vector of  4 elements if the ML model has 4 layers. The operator $|\cdot|$ calculates the absolute value of the vector elements. The output $difference$ is a vector where each element represents the difference of a layer among $N$ models.

As mentioned previously, there are two reputation and FedAvg mechanisms and both of them will be used in the simulation. The first mechanism is "\texttt{HalfFedAvg}" described in Equation \ref{eq:HalfFedAvg} and "\texttt{Reputation-0.05}" described in Equation \ref{eq:Reputation_0.05}.

Because the DFL network is a new computing architecture and we observed many unexpected behaviors and phenomena that never exist in normal federated ML, we present the accuracy and weight difference results from all combinations of non-I.I.D. cases and malicious cases \footnote{the configuration file of each combination is available in \href{https://github.com/twoentartian/DFL/tree/main/paper_result/non-iid-malicious-10nodes}{https://github.com/twoentartian/DFL/tree/main/paper\_result/non-iid-malicious-10nodes}. Notice that for non-I.I.D. cases described by the Dirichlet distribution, there are 10 simulation output folders, and each of them contains a configuration file and a plot of accuracy and weight difference. The subplot in Figure \ref{fig:simulation_whole} in this paper is the average of all plots in the corresponding output folders.} in Figure \ref{fig:simulation_whole}. Table \ref{tab:whole_plot_location} summarizes all combinations of non-I.I.D. and malicious cases and corresponding subplot locations in Figure \ref{fig:simulation_whole}. For example, subplot 13 is located at column 2 and row 4 in Table \ref{tab:whole_plot_location}, "(column 2, row 4)" also represents the subplot location in Figure \ref{fig:simulation_whole}. Each subplot has two parts: part a is the accuracy graph, and part b is the model difference among all nodes.

\begin{table}[h]
\centering
\caption{The subplot location for Figure \ref{fig:simulation_whole}}
\label{tab:whole_plot_location}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
 & IID & \begin{tabular}[c]{@{}l@{}}non-I.I.D.\\ alpha=1\\ (10 repetitions) \end{tabular} & \begin{tabular}[c]{@{}l@{}}non-I.I.D.\\ alpha=0.1\\ (10 repetitions) \end{tabular} & \begin{tabular}[c]{@{}l@{}}non-I.I.D.\\ 1node2labels\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}no malicious\\ HalfFedAvg\end{tabular} & Subplot 0 & Subplot 1 & Subplot 2 & Subplot 3 \\ \hline
\begin{tabular}[c]{@{}l@{}}dataset poisoning\\ HalfFedAvg\end{tabular} & Subplot 4 & Subplot 5 & Subplot 6 & Subplot 7 \\ \hline
\begin{tabular}[c]{@{}l@{}}model poisoning\\ HalfFedAvg\end{tabular} & Subplot 8 & Subplot 9 & Subplot 10 & Subplot 11 \\ \hline
\begin{tabular}[c]{@{}l@{}}no malicious\\ Reputation-0.05\end{tabular} & Subplot 12 & Subplot 13 & Subplot 14 & Subplot 15 \\ \hline
\begin{tabular}[c]{@{}l@{}}dataset poisoning\\ Reputation-0.05\end{tabular} & Subplot 16 & Subplot 17 & Subplot 18 & Subplot 19 \\ \hline
\begin{tabular}[c]{@{}l@{}}model poisoning\\ Reputation-0.05\end{tabular} & Subplot 20 & Subplot 21 & Subplot 22 & Subplot 23 \\ \hline
\end{tabular}%
% }
\end{table}

\begin{figure}
    \centering
     \includegraphics[width=\textwidth]{image/whole.pdf}
    \caption{Simulation results for malicious and non-I.I.D. cases (vectorized image, zoom-in for details)}
    \label{fig:simulation_whole}
\end{figure}

Figure \ref{fig:simulation_whole} shows that the accuracy of ML models can reach over 0.9 under non-I.I.D. and dataset poisoning cases after 4000 ticks. The "epoch" concept is not suitable for DFL because all training samples are randomly selected from the training dataset and injected to the DFL nodes. Randomly choosing training data is closer to practice because each node has no information about the dataset of other nodes in a decentralized network. The total data samples trained by the DFL network (10 DFL nodes) is $ \frac{4000 \cdot 64 \cdot 10}{10} = 256000 $ at 4000 ticks, approximately 4.2 epoch for MNIST training dataset. The accuracy variances in the second and third columns seem to be smaller than those in the fourth column because the accuracy plot in the second and third columns is the averaged result from ten repetitions.

Subplot 8 and Subplot 20 show that \texttt{Reputation-0.05} mechanism can prevent model poisoning in I.I.D. cases, but it does not work in non-I.I.D. cases as shown in Subplots 21,22,23. The factors for successfully training models in non-I.I.D. and model poisoning situations include reputation algorithm, network topology, and the dataset distribution of each node. We have not dived too deep into non-I.I.D. and malicious cases because the reputation mechanism is not our focus. The DFL framework provides a reputation SDK to facilitate further research on reputation algorithms. 

There are some other phenomena in these subplots, which we will briefly discuss in this paper. These phenomena can lead to future research topics:

\begin{itemize}
    \item There is only one model in traditional ML systems and federated ML systems, indicating the model weight difference should be zero when a model is sufficiently trained. However, the model weight difference in DFL does not converge to zero but rather converges to a constant value when the model is properly trained. Subplots 8,9,10,11 also show unsuccessful training has lower model weight difference than successful training. In addition, the model weight difference does not constantly decrease during the training process. The weight difference at 4000 tick is even higher than 600 tick in Subplot 0. In other words, the training result of the DFL network is a set of models rather than a single model, and each model has similar accuracy. One of the potential applications of this property is training models whose dataset relates to geographical location. For example, a disease in different continents has different disease behavior, and there are two DFL nodes on each continent. Both DFL nodes should be able to train a model that can best predict the disease based on different disease behavior. For traditional ML systems, the geographical information must be included in the training dataset, but we would not know that geographical information is critical to the model if we do not aggregate all the data.
    
    \item There is a complex relationship between model weight difference and model accuracy, which we are not yet able to describe yet. The complexity is visible in Subplots 15 and 19 which show that the dataset distribution can change the trend of the model weight difference.
    
    \item In Subplots 0, 4, 12, and 16, there are regions where the accuracy plateaus at 0.5 from 500 ticks to 1000 ticks. The length of the plateau regions scales up with the number of nodes\footnote{this result is based on simulations not shown in this paper}, and it can greatly slow down the ML training when scaling to much larger DFL networks, which requires further investigation. %We have found the cause of the plateau regions and the solution to avoid them, which we will explain in a future paper. 
    These plateau regions are one of the reasons we avoid simulating large-scale DFL networks because they will dominate the training performance. 
\end{itemize}

\subsection{The speed ratio of model training and model updating}
This section investigates the trade-off between bandwidth requirements and ML performance. This is done using simulations to explore the impact of the ratio of model training interval over model updating interval on ML performance. The interval of model training is controlled by training batch size and data injection rate. For example, injecting 64 training samples per 10 ticks with a training batch size of 64 results in one training iteration per 10 ticks. The interval of model updating is controlled by FedAvg buffer size, the number of peers, and the training interval of peers. 

A new node type called "observer" is used in this simulation. The observer node does not train ML models and only performs FedAvg on received models. The observer can ensure that there are enough communications among nodes and that the final model is a combination of training and updating rather than an independently trained model.

Some modifications \footnote{the configuration files are available in \href{https://github.com/twoentartian/DFL/tree/main/paper_result/update_train_ratio}{https://github.com/twoentartian/DFL/tree/main/paper\_result/update\_train\_ratio}} are made to the configuration in Section \ref{subsection:ml_propertires}: 1) simulations use a fully-connected 10-node DFL network; 2) each node uses an I.I.D. dataset; 3) the first node is configured as an observer; 4) the reputation algorithm is "\texttt{Reputation-0.05}". Because the training interval is kept as 8 to 12 ticks, and each node should get 8 models in approximately 10 ticks, we set the FedAvg buffer size to 32, 8, and 2 to achieve different update/train ratios (1:4, 1:1, and 4:1). The result is shown in Figure \ref{fig:simulation_update_train}.

\begin{figure}[h]
    \centering
     \includegraphics[width=\textwidth]{image/update_train.pdf}
    \caption{Update/train ratio simulation results (update/train = 1:4,1:1,4:1)}
    \label{fig:simulation_update_train}
\end{figure}

Figure \ref{fig:simulation_update_train} indicates that more communication among nodes can accelerate the training. It is a trade-off between training speed and bandwidth because more communication requires more bandwidth consumption. We also test several extreme situations where the update/train ratio is 1:32 and the dataset distributions are I.I.D., alpha=1 and alpha=0.1, as shown in Figure \ref{fig:simulation_update_train_1_32}. The third subplot shows that the accuracy has already increased but needs more communication. Figure \ref{fig:simulation_update_train_1_32} shows it is possible to train a model with low-frequency communications, such as in embedded systems and mobile systems.

\begin{figure}[h]
    \centering
     \includegraphics[width=\textwidth]{image/update_train_1_32.pdf}
    \caption{Update/train=1:32 simulation results (I.I.D., alpha=1, alpha=0.1)}
    \label{fig:simulation_update_train_1_32}
\end{figure}


==> Yongding_Tian_DFL_ACM_Revision (Copy to Arxiv) (1)/security_analysis.tex <==
\section{Security analysis}
\label{security_issue}

In this section, we discuss a number of attack methods~\cite{enthoven2020overview, enthoven2021fidel} that can be used by malicious nodes and how DFL can protect against them.

\subsection{Model poisoning attacks}

The DFL system by design is able to defend against  model poisoning attacks by gradually decreasing the reputation of malicious nodes. Ideally, the attack can be fully neutralized when the reputation reaches its lowest point. This process may take time.
% The DFL system should be able to prevent the model poisoning attack by gradually decreasing the weight of malicious node. The attack can be fully neutralized when the reputation reaches the lowest point once the weight becomes zero at lowest reputation point. However, it requires time to figure out the malicious node and decreasing its reputation.

Another potential risk for DFL is that the reputation system might fail once the model poisoning attack succeeds, because the victims cannot generate a model with better accuracy. The reputation system may become "blind" to the malicious nodes because all nodes are producing similar models with similar poor quality. However, it is almost impossible for attackers to compromise all nodes; in this situation, the network can gradually recover by correcting the nodes at the edge of compromised nodes because the innocent nodes can create better-accuracy models.

% Another risk point for DFL is the reputation system might fail once the model poisoning attack succeed because the victims cannot generate a better-accuracy model. For this situations where all nodes cannot create a better ML model, the reputation system cannot find the attacker because all models look similar. However, it is almost impossible to compromise all nodes, in this situation, the network can gradually recover from the edge of compromised nodes because the innocent nodes can create better-accuracy models.

\subsection{Data poisoning and server attacks}
Data poisoning attacks are similar to model poisoning attacks. Both of these attacks can be prevented by decreasing the reputation of the malicious node.

On the other hand, traditional server attacks can be completely prevented because there is no central server in DFL. The ML model on a node is generated by the node itself rather than receiving the crafted models from the server.

\subsection{Model duplication attacks}
\label{model_duplication_attack}
Model duplication attacks are a new attacking method which only exits in blockchain-based federated ML systems. The attack method can be described as an attacker that duplicates the model from other innocent nodes and generates a new transaction with the duplicated model to gain contributions. Verifying the digest of a transaction does not help because the attacker can slightly modify the model weights to get a completely different digest while retaining similar accuracy. 

There are two mainstream solutions to this attack. One is to use Trusted Execution Environments (TEEs) \cite{blockchain_TEE} on all nodes to protect the model data. The other way is to use homomorphic encryption \cite{cloud_homomorphic_encryption} to encrypt the model, which allows other nodes to use the model without decrypting it.

Future versions of DFL will integrate these solutions to prevent these types of attacks. %since it is still at the prototype level.  

% Model duplication attack is a new attack method which only exists in blockchain federated machine learning system. The threat model can be described as the attacker duplicates the model from other innocent nodes, and generate a new transaction with the duplicated model to gain contributions to the model. Verifying the digest of transaction does not solve it because the attacker can slight modify the model weights to get a completely different digest and retain similar accuracy. 

% There are two mainstream solutions to this attack, one is use Trusted Execution Environments (TEEs) on all nodes to protect the model data, another way is using homomorphic encryption to encrypt the model and allow other nodes to use it without decrypting it.

% However, DFL integrates neither of above solutions since it is still at the prototype level. 

==> blockchain_and_machine_learning.tex <==
\section{Blockchain and federated machine learning}
\label{blockchain_and_federated_machine_learning}

This section discusses the design principles of the DFL system and the inspiration behind it. Meanwhile, this section also provides a comparison between DFL and traditional federated ML systems on blockchain. The DFL implementation in Section \ref{DFL_framework} includes more detailed considerations and technical information, while this section only provides the key theory to build a high performance ML system on blockchain.

\subsection{Partial consensus}
\label{partial_consensus}

As previously mentioned, most blockchain systems keep a global consensus. This consensus is essential for a ledger system since miners must validate new transactions based on the current state of each account. Assume two transactions take place in a very short time interval, which are then broadcast to two different nodes quite remote in the network. In this situation, miners would only treat the first received transaction as valid, resulting in different accepted transactions for different miners. But in the blockchain system, only one miner can generate a block which only validates one certain transaction. So the global consensus is critical for the ledger system.

In contemporary cloud computing systems and cloud storage systems, the global consensus is achieved by a centralized server.

However, for ML applications, the global consensus would not be necessary for two reasons. First, the arriving order of transactions is not critical as a late arrived transaction can also be used due to the high tolerance of FedAvg. Second, the model weights in transactions are not critical. Two models might have exactly the same accuracy provided the same test dataset, but their model weights do not necessarily have to be the same.

As discussed in Section \ref{intro_blockchain_system}, global consensus is the cause of bifurcation and contemporary blockchain systems increase the block interval to avoid bifurcation. Nonetheless, the DFL system uses partial consensus rather than global consensus to build a high performance blockchain system for federated ML.

Partial consensus indicates that the models stored in a limited range of nodes should be similar to each other. From the view of network distance, the closer the nodes are, the more similar the models should be. In practice, partial consensus means that the models are only broadcast for a limited distance. All nodes having received this model should take the received model into the next FedAvg iteration. Partial consensus could be an efficient choice because each node does not wait for a global block, which means the traditional synchronized blockchain systems become asynchronous systems. 

Few distributed systems apply partial consensus because of the necessity of a global state. However, as mentioned before, a global state is redundant for machine learning systems. The blockchain database hence becomes the proof of behavior to the contribution of the owner to the model. The proof of behavior in the blockchain also implies the need of having a witness to verify the behavior during the block generation process. In DFL, the witness is the set of neighbors in the p2p network. Neighbors can give feedback on the quality of models by providing the model accuracy based on their own dataset.


Partial consensus can also introduce new vulnerabilities, such as the potential for malicious behaviors like model poisoning to go unnoticed in the network. To address these issues, a reputation system will be introduced in the next section.

% However, partial consensus also brings new vulnerabilities because malicious behaviors, such as model poisoning, can easily hide themselves in this network. So a reputation system will be thrown out to deal with them in the next section.

\subsection{Distributed reputation and weighted federated averaging}
\label{reputation}

The global consensus in a traditional blockchain system ensures no malicious node would dominate the next block, unless they take over more than half of the computation power, called a 51\% attack \cite{blockchain_51_attack}. However, partial consensus allows for malicious behavior such as model poisoning where attackers could easily hide themselves in this network, resulting in new vulnerabilities in the system. A reputation system will be introduced as part of the training ML process to deal with this problem.

There are already some existing reputation systems in the federated ML area. For example,  \cite{reputation_incentive_mechanism} proposed using reputation as an incentive mechanism. The reputation system in DFL is responsible for distinguishing the malicious node in partial consensus. A malicious node can be a node frequently broadcasting low accuracy models, or performing a data poisoning attack or a model poisoning attack. The reputation is distributed and different nodes may rate the same node independently. For example, considering a three-node system - the reputation of node C in node A might be different from that stored in node B. 

The reputation can be updated according to any rational machine learning model criterion. In this paper, we mainly consider updating the reputation according to the model accuracy. More specifically, each node will have its own local reputation record of its neighbors and will update the reputation record based on the accuracy for neighbors' models calculated by itself based on its local dataset. Broadcasting models with higher accuracy earns the node higher reputation in the system. The reputation will be stored locally and not shared with other nodes. 

To protect the system, a malicious node should have a lower reputation in the reputation system. Meanwhile, the influence of malicious models should be lowered as well. We propose using the weighted federated averaging method \cite{weighted_fedavg}, a modified version of FedAvg, in this paper. The modified FedAvg mechanism works together with the reputation system to keep the federated ML secured and stable.


In Section \ref{result_and_discussion}, we implement a sample reputation and weighted average system. However, more factors should be considered for a more universal implementation. These factors include but are not limited to the malicious rate (proportion of malicious node), training performance (the accuracy curve), the data distribution (non-I.I.D. dataset). The variances in these factors will lead to quite different implementations of reputation and weighted FedAvg system. 

DFL is designed to be flexible towards the above variations, such as different dataset distribution, malicious rate, network topology. The reputation implementation and new federated averaging algorithm can be dynamically linked to the DFL framework, while basic tests are performed to ensure the correctness of external reputation and weighted federated average implementation.

\subsection{The blockchain database}
\label{the_block_chain_database}

In traditional blockchain systems, the blockchain database stores all verified transactions and all miners need to process the transactions on the blocks. However, in a partial consensus system, there is no such unique blockchain database, otherwise the system will fall back to a global consensus and struggle with bifurcation. 

In DFL, the blockchain database works as a proof of contribution. The generator needs to generate a block recording the contribution in model training. These contributions should be able to be verified by external nodes in the network. The verification results will be appended to the block forming a final block, whose digest will be used to generate the next block.

With this method, the generator cannot modify the blockchain database because there is no chance to get a second verification. The previous block also cannot be modified as each block is chained by the digest. This property corresponds to the immutability of traditional blockchain.

Though blockchain database is a proof of contribution, it is not a measure of contribution. In traditional blockchain systems, miners can get tokens as rewards for their participation in consensus. In a federated ML system, nodes should be able to get rewards if they trained the model based on their own data. However, the reward is not measured by the amount of transactions (models) in the blockchain database. The reward should be the mixture of reputation and blockchain database. The algorithm to calculate reward, based on blockchain data and reputation, is not covered by this paper. 

==> response.tex <==
\newpage

\section{response to reviewer's comments}

I am sorry that I submitted the response to 1st-round reviewers' comments in the Latex source files, so no 2nd-round reviewer read it.

\subsection{2nd round of revision}

\textbf{Regarding the issues in Figure Simulation results for malicious and non-I.I.D. cases}

\textbf{Reviewer: reduce (or split in different figures) the number of plots in figure 13, logically split Section 5.2 into sub-sections, dividing the explanation of the results of the experiments}

\textbf{We have increased the font size for a better reading experience. Regarding the suggestion of splitting the figure, we discussed it together and would rather not split the figures because of the following reasons: (1) the font size is limited by the number of columns. If we reduce the number of columns, the figures would be harder to compare because we want to compare the accuracy and model weight difference (Y axis) (2) the conclusion in the simulation part is to show that DFL is possible to work in these situations and opens more research topics. Considering that our contribution is not reputation/rewarding algorithms, we'd rather not split its discussion into multiple parts. (3) Table 9 is useful for understanding Figure 89 because it shows the location of the subplots and the meanings of each location. }

\subsubsection{Reviewer 1 (2nd revision)}
\textbf{\#\#\# The design of partial consensus is not clear. A figure could be used to present the partial consensus mechanism.}

\texttt{Partial consensus is moved to Section 3.1. Now "Gossip algorithm" is added to the partial consensus section because it is similar to the idea of partial consensus. The gossip algorithm should be easy to understand because there are already many research papers about it. Introducing the Gossip algorithm first should also clarify the partial consensus.}


\textbf{\#\#\# How are the hyperparameters chosen in this work?}

\texttt{we directly use the hyperparameters in Caffe Lenet to avoid ML-side issues, "We use the same hyperparameters as the LeNet example in Caffe"-Section 5 Result and discussion, 1st paragraph.}


\textbf{\#\#\# To improve the quality of this work, the author should reorganize the structure of the paper, especially for Section 3 and Section 4.}

\texttt{Section 3 and Section 4 are reorganized as suggested by Reviewer 2}


\subsubsection{Reviewer 2 (2nd revision)}
\textbf{\#\#\# In fact, this shows up in Section 5, which needs to  separate the experimentation from the simulation part (the latter stripped of blockchain functionality) I think it would have been fruitful to first prove that the decentralised FL scheme works and in follow-up work, introduce the blockchain-based incentive mechanism}

\texttt{The paper first shows the experimentation because only experimentation can show the resources consumption and further prove our initial motivation: DFL has better performance than existing blockchain-based FL systems, just as the title suggests. Another reason is that experimentation only has 2 or 4 nodes, which is simpler than the 10-node simulations.}

\texttt{Regarding this suggestion "first prove that the decentralized FL scheme works and in follow-up work, introduce the blockchain-based incentive mechanism", our initial thinking is "first show DFL is working (a least in small scale networks) and scaling up to larger networks". However, due to deployment issues and code stability issues, we failed to scale to larger networks, so we turned to using simulations. In addition, we know our decentralized FL scheme, unfortunately, cannot work properly in large-scale networks (50 nodes or above), so I'd rather not use the simulator to "prove" our scheme.} 


\textbf{\#\#\# Key insights may be given by the literature on gossip FL and graph neural networks, but they are not mentioned in the paper (see 3d).}

\texttt{Gossip FL literature is added to Section 3.1 and compared with DFL in Section 3.4}

\textbf{\#\#\# however they are missing very relevant works in the areas of "decentralised FL", "gossip FL", and even "assisted learning". For example,
Pappas, Christodoulos, et al. "Ipls: A framework for decentralized federated learning." 2021 IFIP Networking Conference (IFIP Networking). IEEE, 2021.
replaces the server in FL with a decentralised network, offers a concrete implementation, and is asynchronous. The only distinction is that it uses IPFS instead of blockchain. Its Related Work section (Sec 4) is also highly relevant: see for example
Roy, Abhijit Guha, et al. "Braintorrent: A peer-to-peer environment for decentralized federated learning." arXiv preprint arXiv:1905.06731 (2019).
You will find other works with the keywords that I mentioned above. I would recommend adding a paragraph or two in the introduction discussing / comparing with these solutions}

\texttt{These publications are added to Section 3.1, Section 3.4 and the reference list}


\textbf{\#\#\# Why is blockchain needed in FL? (To remove the server, which is a single point of failure and potentially malicious, offer convenience to developers etc). Has it been done and what were the limitations? (has been tried on public blockchains but is costly, ineffective due to the latency, storage hungry etc.. also a comment on gossip learning and other solutions like in 3d) What does this paper propose and why is it better?}

\texttt{Add two paragraphs in Introduction}

\textbf{\#\#\# I would describe the reputation system in section 4 or even better section 3 as it is really part of the proposal.}

\texttt{DFL provides an interface to design various kinds of reputation algorithms and federated average algorithms, so the reputation algorithm in our paper is just an example of the interface and we don't wish to put it in our major contributions.}

\texttt{In addition, I know there are many limitations in our reputation algorithm and I personally believe it will soon be replaced in the future.}

\textbf{\#\#\# Links to Github should be footnote}

\texttt{Fixed}

\textbf{\#\#\# for the Dirichlet distribution, I would write "For the non-IID samples, we sampled a probability distribution over the class labels for each node based on a symmetric Dirichlet prior. In particular, we investigated the cases a=1 and a=0.1 where  a is a concentration parameter of the Dirichlet distribution meaning etc"}

\texttt{Fixed in Section 5.2}

\textbf{\#\#\# I guess the division with the random numbers refers to \newline https://en.wikipedia.org/wiki/Dirichlet\_distribution\#From\_gamma\_distribution, is that correct?}

\texttt{yes it's correct}

\textbf{\#\#\# please clarify eq 7, Is difference a vector or scalar? is N the number of nodes (one model per node) or the models in the buffer? why sum the weights for each layer and not take the vector difference?}

\texttt{The difference is a vector and each element represents the difference of a layer, the N is the number of nodes/models. Summing the weights of a specific layer in $Model_n$ (because a layer may have thousands of weights) results in a value, and we use that value to represent the layer. So a 4-layer network has 4 vector elements in $Model_n$}

\textbf{\#\#\# There are too many subplots in Fig. 13 and they are rendered so small that they cannot be read. In my opinion, this section should be broken in cohesive units (for example, subsections on no malicious, data poisoning, model poisoning attacks). Now the data generation methods, threat model and evaluation metrics are all mixed together.}

\texttt{I increased the font size of the figure and it should be better now. We would rather not split the figures because (1) the current form is easier to compare and (2) there are many cross-figure analyses in the following part and (3) splitting the figures may exceed the page limitation}

\textbf{\#\#\# usage of "extremely"}

\texttt{Fixed}

\textbf{\#\#\# a reputation system will be "thrown out" to deal with them}

\texttt{Fixed}

\textbf{\#\#\# "high/low performance" is generic, better state directly the metric, e.g., "low latency / accuracy"}

\texttt{Fixed}

\textbf{\#\#\# possibilities should be probabilities (for the Dirichlet distribution)}

\texttt{Fixed}

\textbf{\#\#\# one sentence paragraphs should be avoided}

\texttt{Fixed}


\subsubsection{Reviewer 3 (2nd revision)}

\textbf{the new results section sounds quite confusing (in particular the simulation with non i.i.d dataset and malicious user). In my opinion, the authors should organize the results section in order to make it easier to read and understand. I recommend adding a threat model so that the reader can easily understand the strengths and weaknesses of the DFL framework.}

\texttt{I re-organized the paragraphs in simulation section to make it more clear.}

\texttt{There is an explanation about how attacks are performed in simulation section (5.2) paragraph 3: "There are two types of malicious nodes..."}

\texttt{The simulation section is not meant to illustrate the strength or weakness of DFL. The strength of DFL is that it allows asynchronous ML training in a p2p network with distributed blockchain as a proof of contribution. The weakness is that it makes dataset/model attacks easier so we introduce a reputation system. Section 3 (High-Level overview of DFL) presents similar points. }

\textbf{In the new section 4.4, the authors propose some applications of the DFL framework. My main concern about these applications is that all of them rely on the existence of an incentive mechanism even if it is not part of the contributions of the paper. Several issues may arise in the definition of incentive mechanisms. In my opinion, section 4.4. could be defined as a "future work" considering that it does not present any real-world application for the current version of the DFL.}

\texttt{I agree it's not decent to call them "Applications", so I changed the title from "Applications" to "Possible applications" and added a sentence to tell readers these applications are only feasible with proper reputation algorithm and federated average algorithm.}

\textbf{the choice of incentive mechanism is crucial to fill the "lack of motivation" issues. Considering that the motivation behind the use of blockchain technology is mainly due to the proof of contribution, several issues, about the entity (or entities) responsible for the assignment of incentives, arise.}

\texttt{I agree that there are many blank areas in the reputation and rewarding systems, and the solutions to these issues are application-specific (selection of responsible entity). The blockchain database in DFL is just a proof of contribution to ML models (models are shared with other nodes), it doesn't measure how much contribution is made.}

\textbf{reduce (or split in different figures) the number of plots in figure 13, logically split Section 5.2 into sub-sections, dividing the explanation of the results of the experiments}

\texttt{Please refer to the beginning of the response (2nd revision)}


\subsubsection{Reviewer 4 (2nd revision)}

\textbf{Using the accuracy as a means of computing the reputation of a node does not foster appropriate learning in the face of non-i.i.d. settings. Also, it does not allow to discriminate whether the low accuracy is due to the node being malicious, or having insufficient local data during the learning process}

\texttt{I agree that the current accuracy-based reputation/FedAvg algorithms cannot discriminate malicious and non-i.i.d. nodes. However, there are some misunderstandings about nodes with insufficient training data. Nodes that have insufficient local data for training, will generate fewer transactions and generate fewer blocks, thus getting less reward for model contribution. They can still catch up with the main net if they constantly do model averaging (relevant to the observer concept in Fig 11), and do no harm to the global model. }

\texttt{For extreme non-i.i.d. nodes (e.g. nodes that have training data that no other nodes have, or the training data is so rare that no neighbors can confirm the model contribution), their difference from malicious nodes requires further research.}

\textbf{The article is missing an in-depth analysis to validate one fundamental claim: “this architecture achieves extremely high performance with low resources consumption by waiving global consensus”. In my opinion, this claim should represent the main scope of the article and is currently weakly supported. In order to strengthen its validation, the authors should deepen the DFL performance section by either: Performing experiments that evaluate the DFL performance should also be supported by a comparison with a federated process run under different blockchain systems (e.g., time to reach the same accuracy in the scenario, time needed by each node to perform its own operation under different systems)}

\texttt{I added two paragraphs in Section 5.1 (Result and Discussion - DFL performance) to roughly compare DFL with BAFFLE in terms of execution time. The major difficulty in comparison is that most blockchain-based FL projects are based on simulations and seldom of them have deployment results (blockchain-based FL has become popular yet, either). For projects with deployment results, our test methods are also significantly different. e.g. BAFFLE first trains a global ML model and then records the ML procedures on the blockchain, while in DFL the two processes happen simultaneously. The BAFFLE performance is limited by chunk size(a smart contract parameter), which is, however, just an engineering limitation (because the smart contract concept is not originally designed for ML activities).}

\textbf{However, since the scope is to propose an underlying system based on blockchains, the experiments on the DFL performance are rather poor, and the quality of the system is not properly highlighted by a comparison with other existing blockchain-based systems.}

\texttt{I would like to append some comments after the previous response to "The article is missing an in-depth analysis to validate one fundamental claim...". The major reason for "DFL has higher performance than other projects" is that it releases the blockchain restriction, allowing nodes to do ML activities without waiting for a block to be finalized. In the new submission, Section 3 (High-level overview of DFL), the first paragraph, briefly describes it and Section 4 shows the technical details to show its async property. }

\subsection{1st round of revision}

\subsubsection{Reviewer 1 (1st revision)}

Thank you for your suggestions

\textbf{\#\#\# My main concern for the paper is the actual need for blockchain technology. In general, the blockchain enforces a global state among many nodes in a decentralized manner but, in the proposed solution, each node maintains a separate blockchain that records the transactions related to that particular node. Why is immutability needed in this case? More specifically, it is not clear from the text how the receipts from other users are used. According to my understanding, there are 2 types of accuracies: (1) accuracies for the node's model calculated by neighbors, and (2) accuracies for the neighbors' models calculated by the user. The accuracies from (1) cannot be used as reputation because the other nodes may have faked them, so why are they recorded?} 

\texttt{Thank you for your concern. I realized that I didn't explain the role of the DFL blockchain data. The blockchain data is proof of contribution to ML models. Model designer/company/smart contract can distribute rewards based on this proof and reputation (in other words, it is an incentive mechanism). The "Figure 1 DFL overview" in the revision explains this process and the "DFL framework - Applications" section (changelist 3) gives several examples of using the blockchain data as incentive mechanisms.}

\texttt{It's possible that some malicious nodes will give false accuracies (1) to model generators, causing inaccurate reward distribution. We haven't done any research on it but it should not be big trouble because most nodes should be innocent.}

\texttt{Because the blockchain data is a proof stored on the node's machine, it should be immutable, otherwise, a node can easily discard previous information in the blockchain data and causes inaccurate reward distribution.}

\texttt{The first use of receipts is calculating the contribution to the ML model. The accuracy (1) is immutable before generating a block otherwise the node will not get block confirmation. After generating the block, the accuracy (1) is also immutable until the blockchain data is submitted to the rewarding system.}

\texttt{The rewarding system can be a centralized server if the ML model owner is a commercial company. Or a smart contract on a traditional blockchain system if the ML model is driven by the community. The interval of submitting blockchain data can be relatively long (e.g. one month) to reduce the load.}

\texttt{The accuracy (2) is used to update reputation and update models.}


\textbf{\#\#\# What if the selected neighbors have insufficient data for good training? How can the TTL be adapted?}

\texttt{In DFL, we have a special node type called "observer" node, which only receives and averages models from others and never train the model. This role is used to prevent the case that all nodes can have good accuracies if each node uses IID dataset and self-training dominates the model (which means they seldom share their models).}

\texttt{In result section, "5.3 The speed ratio of model training and model updating", there are some simulations about an observer node.}

\texttt{Observer nodes won't contribute to or damage the global training process, nor generate blockchain to prove his contribution.}

\texttt{TTL is not related to observers here. The TTL is designed to do trade-off between "model broadcast speed" and "network consumption". Larger TTL can let the models broadcast faster but causes larger network flood. }

\textbf{\#\#\# What if the neighbors do not reply, e.g., because of network failures?}

\texttt{There are three cases:}

\texttt{ - Node A fails to send model to Node B: Node A will remove Node B from peer list. This case won't affect the blockchain data.}

\texttt{- Node A sends model to Node B but doesn't get a receipt: The receipts from Node B will be missing in the blockchain file of Node A. But it doesn't matter for Node A because there are other neighbors to proivde receipts.}

\texttt{- Node A sends model to Node B and receives receipt, but fails to send block to Node B or doesn't receive block confirmation. Node A is allowed to finalize the block once he collects enough block confirmations (for example, 80\% of receipts are confirmed). So network failure on a few peers won't bother the blockchain process.}

\textbf{\#\#\# How do the users coordinate to start a training task?}

\texttt{This is a very good question. The answer might sound counterintuitive.}

\texttt{The answer is: coordinations among nodes will slow down the training process (the accuracy grows up much slower). Coordination includes: nodes start training with the same dataset; nodes start training at the same time (and all nodes have the default random model).}

\texttt{There is a special phenomena behind DFL (also applies to all ML systems if they use a similar partial aggregation) and it's not obvious for small size network. For DFL network with over 50 nodes, the phenomena will dominate the training curve. This is also one of the reasons that we don't hope to mention large DFL network because there are too many things to discuss.}

\texttt{If you are interested, you can find the phenomena here\footnote{https://github.com/twoentartian/DFL/blob/main/readme/2021-09-29\%2015:05:15\%20GMT\%2050\%20nodes\%2C\%206peer\%2C\%202\%20observer/accuracy.png}}

\texttt{We will not add the this topic in this paper because it relates to some unpublished work.}

\textbf{}{\#\#\# A comment on the communication cost would be appreciated. For example, could the neighbors return receipts directly instead of flooding to save on bandwidth?}

\texttt{It is hard to make comments on the communication cost due to following reasons:}

\texttt{- In traditional FL, we can send gradients to reduce the communication cost. But in DFL, you must send the whole model. (DFL integrates a compression tool to compress the model and evaluate the performance. This paper doesn't mention it.)}

\texttt{- The communication cost depends on the size of ML model, TTL and the number of peers.}

\texttt{The neighbor send the receipts to other nodes because we want to provide an interface for reputation algorithm to utilize the accuracy from other nodes. The accuracy from other high-reputation nodes might be useful.}

\texttt{Of course, DFL is just a prototype, future projects can remove/add components based on DFL. So we choose to keep flooding for a better reputation interface.}

\textbf{\#\#\# Do the nodes perform training for an epoch and then wait for the models of the neighbors or do they keep training? How does that affect the performance if the nodes do not receive replies?}

\texttt{The new "result" section gives detailed explanations on how training and updating models works.}

\texttt{The node will collect enough data (e.g. data size == batch size) and perform training, after training the node will seal the model in a transaction and broadcast the transaction to other nodes. The "epoch" concept doesn't apply in the DFL because we will never know the complete dataset.}

\texttt{In experiment, the data is randomly selected from MNIST dataset. In simulation, the data is randomly selected with specified distribution. (the distribution is available in the simulator configuration file)}

\texttt{The node will not wait for other nodes. The node only needs to perform model updating when collects enough transactions. The training phases on different nodes are completely asynchronous. Of course the node also needs to generate receipt/block confirmation for other nodes.}

\texttt{The blockchain data is a proof of contribution. It's not a problem if a node sends a transaction to 10 peers but only receives 9 receipts because 9 accuracy feedbacks are enough to characterize its contribution. So missing replies won't influence the performance, it will only make the blockchain proof less accurate.}

\textbf{\#\#\# Do the nodes they wait for their buffer to get filled to average? Do they transmit a model only after an averaging?}

\texttt{Do the nodes they wait for their buffer to get filled to average - yes}

\texttt{Do they transmit a model only after an averaging - no, they transmit a model after training. Figure  1 clarifies this.}

\textbf{\#\#\# What is the impact of the size of the buffer?}

\texttt{Covered in the new "5 Result" section. "The speed ratio of model training and model updating" subsection.}

\textbf{\#\#\# Regarding the reputation mechanism, a key limitation is that it does not work as-is but needs tweaking. Also, can the reputation be reset? Does it apply only for a specific training session?}

\texttt{The DFL framework provides a SDK for updating reputation and models. In the SDK, you can do anything you want. The major problem for reputation is that the algorithm itself is application-specific (e.g. how many attackers are there, the number of parameters, will the trend of data changes, etc)}

\texttt{Also, can the reputation be reset? \-\- yes, once the algorithm requires.}

\texttt{Does it apply only for a specific training session? \-\-depends how you design the reputation algorithm}

\textbf{\#\#\# The implemented network is too simple for meaningful conclusions about the real-life applicability of the solution: 4 fully connected nodes, which can be reached in 1 hop, hiding the impact of TTL}

\texttt{The 4-node fully-connected network is currently our best effort because the DFL is still at the prototype level. Configuring and running this 4-node network without any bugs is already a not-easy work. }

\texttt{In addition, we know there are some hidden "traps" in large-scale DFL networks.}

\texttt{We performed some simulations on 50/100 nodes DFL network, and we found an interesting phenomenon: 
\footnote{https://github.com/twoentartian/DFL/blob/main/readme/2021-09-29\%2015:05:15\%20GMT\%2050\%20nodes\%2C\%206peer\%2C\%202\%20observer/accuracy.png} }

\texttt{We are currently trying to re-produce this phenomenon in deployment. If everything goes well, a paper will come out to discuss it. After that paper, we will do some research about the impact of TTL (hopefully).}

\textbf{\#\#\# Also, the storage and privacy requirements are mentioned in the Introduction but are not addressed later on. There is no comparison, even ball mark estimates, with literature approaches in terms of throughput, computational and communication load. }

\textbf{\#\#\# \- Merge Sections 3 and 4 since they both refer to the proposed method.}

\texttt{Sorry that I won't merge the two sections for the following reasons:}

\texttt{- From my point of view, Section 3 is a very important section, even more important than Section 4, because it elaborates "how" to design an asynchronous \& high-performance ML system on blockchain.}

\texttt{- The DFL framework in Section 4 includes too many unnecessary considerations and technical details (e.g. flooding the accuracy measured by neighbors to other neighbors). Future researchers might have better mechanisms to generate blocks (e.g. without using two communication rounds in generating a block).}

\texttt{- If I merged Section 3 and 4, readers need to think and summarize what is important and what can be discarded.}

\textbf{\#\#\# There is no comparison with other methods in the experimentation section, which is partly justified because the solution is not directly comparable. Nevertheless, there should be at least an approximate analysis of the throughput, latency, and storage benefits of the proposed method, which was the initial motivation.}

\texttt{I mentioned the storage benefits in "4.5 Considerations and comments".}

\texttt{As for the "throughput" and "latency", in traditional blockchain,  "throughput" is how many transactions we can process per second and the "latency" is how many seconds we need to wait until the transactions appear in the block. I don't think these two concepts exist in DFL because the DFL transactions will not reach all nodes. The "latency" also doesn't make a lot of sense for us because DFL is an asynchronous system. It does not matter whether this node is performing machine learning or block generation.}

\texttt{We investigate the blockchain overhead because less blockchain overhead is always desirable.}

\subsubsection{Reviewer 2 (1st revision)}

Thank you for your suggestions

\textbf{\#\#\# The quality of writing of the manuscript may be definitely improved. The discussion of the methodology is quite confusing. Section 3 is full of go-to-sections and, instead of providing the actual design principles as stated by the authors, it seems to be an informal discussion of what is defined in Section 4. The latter instead, which describes the framework, is too concise and it does not highlight in a clear way how the proposed method differs from traditional blockchains. A good way to address these issues could be to merge the two sections, and provide the right amount of both technical details and informal discussion, to allow the reader to get context and the impact more easily. The formatting of these sections does not help: the figures are quite detached from the context they refer to.}

\textbf{\#\#\# Concerning the contributions to FL, the scope of the article is not stated. FL spans on a wide range of applications, from cross-device to cross-silo, which are much different in terms of functional and non-functional requirements. The authors should clarify what are the contexts in which this methodology can be applied.}

\texttt{In fact, I'd rather not use traditional FL terms or concepts because the FL part in DFL is too different from traditional FL. The absence of a global model and updating with partial aggregation of models make the DFL unique in ML area. I still use "FL" in this paper because many algorithms such as FedAvg can be directly ported to DFL, and these two systems share many ML properties. }

\texttt{As for "cross-device" or "cross-silo", I think DFL can work for both types.}

\texttt{Cross-silo: Section "5 RESULT AND DISCUSSION" simulates a non-IID case where each node only has data samples with 2 specific labels.}

\texttt{Cross-device: I don't think "cross-device" can efficiently describe DFL  because there is no "training round" in DFL. For cases where only small portion of nodes can send models to other nodes, Fig 15 indicates (but not prove) that DFL can work properly with limited model broadcasting.}

\texttt{The DFL blockchain system might not work if all nodes frequently go online/offline in cross-device cases, but the ML side can work properly with a broker to temporarily store and forward the models. }

\textbf{\#\#\# The choice of the update rule for the model aggregation is completely wrong. Evaluation of the received model on a local dataset to measure the accuracy and, consequently, the reputation of another node for weighting the contribution of the model to the update misses the main point of federated learning: learning a global model, or increasing the local performance in the face of lack of data.}

\texttt{I am not sure I understand what's your concern here because, from my point of view, the model aggregation in DFL is completely from FL (Section 3 and Section 4 have already shown the DFL mechanism), and the model update rule in DFL of course will miss the main point of traditional FL.}

\texttt{By the way, I would like to address that there is no "global model" in DFL. }

\textbf{\#\#\# With the use of this aggregation rule, models which work on a different local distribution (which may be the more informative), are penalized by the statistical heterogeneity, instead of taking advantage of it. }

\texttt{Models working on a more informative dataset should have higher accuracies on the other nodes' dataset and take more weight in the other nodes' updating process. The model generator can record these accuracies in blockchain as proof of contribution.}

\textbf{\#\#\# Furthermore, there is no mention about how the evaluation dataset is designed, which brings me to the last point.}

\texttt{The new "result" section explains how test dataset is selected. The test dataset in experiment is randomly selected from all received data samples. The test dataset in simulation is randomly selected from the MNIST test dataset.}

\textbf{\#\#\# The experimental assessment has too many blind spots. There is no mention about how the data was split between nodes, what is the “test set” where the local models are evaluated (is it a local split of the data? An external global dataset?), how many training epochs a node performs before starting the transactions. }

\texttt{Thank you for your suggestion. I re-wrote the whole "result" section, and this version contains a detailed deployment configuration. The configurations for simulation are also open-sourced on Github, and there will be direct links to them.}

\texttt{In the experiment, all nodes get a certain amount of samples randomly selected from the MNIST dataset every second (different data samples for different nodes). Each node performs training once the received data >= batch size and broadcasts the trained model to other nodes. We don't use epochs anymore because nobody knows what's the whole dataset in a p2p network.
In the revision, the new "Section 5 Result" should clarify this point.}

\textbf{\#\#\# Also, the experiment depicted in section 6.5 seems to hide a crucial point of what I mentioned before about the aggregation rule. If the data is i.i.d. across 4 clients, while there is a malicious node, it seems naïve that the other nodes’ models will be ranked higher: their learning process is proceeding on approximately the same distribution, and they will perform well on each of the others’ local datasets. But what happens if the data is non-i.i.d. across clients and the guarantee of the malicious node being ranked lowest comes less? This should be investigated, too.}

\texttt{I hope Section 5.2 and Fig 13 in revision can answer this question. In non-I.I.D. + dataset poisoning cases, the model will be trained slower but still reaches an acceptable accuracy. In non-I.I.D + model poisoning cases, you are correct that there is no guarantee that the malicious node will be ranked lowest. We need more complex reputation algorithms to identify malicious nodes and non-IID nodes. The sample reputation algorithm is only used to prove the DFL framework works, and it's not our major contribution. The major contribution of this paper is solving the performance issue in traditional ML on blockchain systems by asynchronizing the blockchain and ML. }

\textbf{\#\#\# Finally, in table 5, experiments show a huge overhead given by the blockchain system (and by the “calculate accuracy” operation for computing the reputation) even with four nodes. Provided that the FL scenarios are inherently massively parallel, I am very skeptical about both the applicability of the framework and the trade-off between costs and benefits in terms of security. Even if the framework allows for a faster update between local nodes, propagating the nodes’ updates to the whole network may still be really costly.}

\texttt{1. The experiment result is CPU time. 1 second means a CPU core runs for 1 second rather than 1 physical second.}

\texttt{2. The time spent on "Calculate accuracy" and "broadcasting" is proportional to the number of peers. And a single node usually only has limited peers. In the revision, we simulate a 10-node network with each node having 4 peers.}

\texttt{3. The nodes’ updates will never be propagated to the whole network. There is an integer called "TTL" in transactions. TTL will be reduced by 1 once forwarded, and the node will stop broadcasting the transaction if TTL reaches 0. Because TTL can be defined in the genesis block and each node has the same "initial TTL" value, it is impossible for a node to broadcast the transaction to the whole network. In our experiments and simulations, the TTL is fixed to 1.}

\subsubsection{Reviewer 3 (1st revision)}

Thank you for your suggestions

\textbf{\#\#\# the authors should add a presentation of the related works. The "RELATED WORK" section only introduces the topics covered in the manuscript without referring to other solutions proposed to solve the integration of the federated learning algorithm in the blockchain technology;}

\texttt{From our limited knowledge, the most-related and widely-applied solution is to integrate federated ML with blockchain technology using smart contracts to do model aggregation and model updating. I have already mentioned it in Section "2.3 Federated machine learning on blockchain".}

\texttt{There are also many blockchain-level acceleration methods, such as layer-2, and side-chain, but they are unrelated to this paper. Mentioning them here might let readers think we will propose a similar thing. However, DFL is fundamentally different from them.}

\texttt{There is also a lot of research about building/optimizing the federated ML on the blockchain on the theoretical level, but no research addresses the poor blockchain performance. Because the DFL framework focuses on performance, mentioning these researches might mislead readers.}

\texttt{As far as we know, there are only two papers (ref 10, ref 17) deploying ML applications on a practical blockchain project, and both of them are mentioned.}

\texttt{BTW, I changed the section name from "RELATED WORK" to "RELATED WORK AND BACKGROUND"}

\textbf{\#\#\# Section 3.4 introduces the reader to the Weighted federated averaging }

\textbf{\#\#\# although the reference [22] describes the FedAdp algorithm. Which algorithm do you use and why? I suggest adding the reasons that led to the choice of the algorithm used.}

\texttt{In the new result section, we give each algorithm a name: "HalfFedAvg" and "Reputation-0.05".}

\texttt{I don't think other papers will mention similar algorithms because they don't need to keep 50\% old models (the old model contributes 50\% of the new model in updating process). DFL needs the old model because the peers is not trustworthy and only "my own model" is trustworthy.}

\texttt{The major contribution of DFL is not FedAvg algorithms and the algorithms are only used to show the DFL works (we add this point in the new "1. introduction" section).}

\texttt{In addition, I don't think there is too much research value in our FedAvg algorithms. I believe future researcher can design something better. }

\textbf{\#\#\# \- It is not clear how the framework set the configuration of the federated learning algorithm (e.g. federated rounds, local epochs, loss function). Considering the algorithm used to define the reputation, it needs several federated rounds to "identify" a malicious user. For this reason, I think it is important to specify the configuration of the federated learning algorithm and, probably, the related assumptions/limitations.}

\texttt{The "result" section has been completely rewritten. And the new "Result" section should answer most of the configuration questions in our simulation.}

\texttt{The configuration files to reproduce the result is open-sourced and you can find the links in the paper.}

\texttt{I can briefly answer it here: we don't use "federated rounds", "local epochs". "local epochs" is replaced by "how many training samples injected per tick". "federated rounds" doesn't exist because it is a kind of synchronization, and DFL is completely asynchronous. The loss function is the original loss function for LeNet/MNIST (sparse\_categorical\_crossentropy).}

\textbf{\#\#\# the experiments involve only one dataset and one model. I suggest extending the experimental evaluations on different datasets (e.g. federated learning benchmark) and different models. It could be interesting to test the framework using simpler models and add a comparison with the results obtained using a traditional ML configuration algorithm. }

\texttt{Thank you for your suggestion. Our develop team will add support for ML models and dataset in the future. Currently we are doing some work about "large-scale DFL network" and don't have extra time to implement interface for other ML models and datasets.}

\texttt{By the way, the major contribution of DFL is the partial aggregation of models and integrating ML with blockchain in an asynchronous way. Supporting more ML models and dataset does not add extra value to our major contribution point, so we can only do it in the future.}

\textbf{\#\#\# the experiment with the Non-I.I.D dataset should show the distribution of the training example among the nodes. It is only specified that the partitions follow a Dirichlet distribution without showing the actual number of examples per class owned by each node.}

\texttt{We didn't do any experiments with the Non-I.I.D. dataset, I guess you mean simulations.}

\texttt{In the new result section, all simulations configurations are open-sourced. We don't directly put the distribution of the training example on the paper because there are too many. You can find a link to these configurations (in Section 5.2 ML properties (simulation).}

\textbf{\#\#\# it is not clear how the FedAvg buffer works.}

\texttt{We added Fig 1 DFL overview and it mentions how model buffer (FedAvg buffer) works.}

\texttt{The result section also describes the model buffer parameters for simulation and experiments.}

\textbf{\#\#\# the DFL supports only the accuracy metric that, in several machine learning tasks, is not a good indication of the model performances. Is it possible to generalize the proposed approach with other metrics? }

\texttt{Thank you for your suggestion. I think our development team will discuss more ML metrics in the future.}

\texttt{During this revision, we add a metric called "model weight difference", which can describe how different the models in the DFL network are. This metric shows many interesting results that require further research.}

\textbf{\#\#\# the structure of the manuscript presents several sections with a short description. I strongly suggest reviewing the structure and flow of the paper by gathering sections in macro-topic with an in-depth description of the topics presented.}

\texttt{We have reviewed the structure, and many small sections have been merged into a large one. Our modifications are based on the suggestions from the first reviewer because he also mentioned this problem.}

\texttt{BTW, I feel like I didn't clarify what are the major contributions of our paper. So I add a paragraph to explain the major contribution in section "1. Introduction". The section "4.4 Applications" also describes some possible applications to elaborate our contribution.}


==> security_analysis.tex <==
\section{Security analysis}
\label{security_issue}

In this section, we discuss a number of attack methods~\cite{enthoven2020overview, enthoven2021fidel} that can be used by malicious nodes and how DFL can protect against them.

\subsection{Model poisoning attacks}

The DFL system by design is able to defend against  model poisoning attacks by gradually decreasing the reputation of malicious nodes. Ideally, the attack can be fully neutralized when the reputation reaches its lowest point. This process may take time.
% The DFL system should be able to prevent the model poisoning attack by gradually decreasing the weight of malicious node. The attack can be fully neutralized when the reputation reaches the lowest point once the weight becomes zero at lowest reputation point. However, it requires time to figure out the malicious node and decreasing its reputation.

Another potential risk for DFL is that the reputation system might fail once the model poisoning attack succeeds, because the victims cannot generate a model with better accuracy. The reputation system may become "blind" to the malicious nodes because all nodes are producing similar models with similar poor quality. However, it is almost impossible for attackers to compromise all nodes; in this situation, the network can gradually recover by correcting the nodes at the edge of compromised nodes because the innocent nodes can create better-accuracy models.

% Another risk point for DFL is the reputation system might fail once the model poisoning attack succeed because the victims cannot generate a better-accuracy model. For this situations where all nodes cannot create a better ML model, the reputation system cannot find the attacker because all models look similar. However, it is almost impossible to compromise all nodes, in this situation, the network can gradually recover from the edge of compromised nodes because the innocent nodes can create better-accuracy models.

\subsection{Data poisoning and server attacks}
Data poisoning attacks are similar to model poisoning attacks. Both of these attacks can be prevented by decreasing the reputation of the malicious node.

On the other hand, traditional server attacks can be completely prevented because there is no central server in DFL. The ML model on a node is generated by the node itself rather than receiving the crafted models from the server.

\subsection{Model duplication attacks}
\label{model_duplication_attack}
Model duplication attacks are a new attacking method which only exits in blockchain-based federated ML systems. The attack method can be described as an attacker that duplicates the model from other innocent nodes and generates a new transaction with the duplicated model to gain contributions. Verifying the digest of a transaction does not help because the attacker can slightly modify the model weights to get a completely different digest while retaining similar accuracy. 

There are two mainstream solutions to this attack. One is to use Trusted Execution Environments (TEEs) \cite{blockchain_TEE} on all nodes to protect the model data. The other way is to use homomorphic encryption \cite{cloud_homomorphic_encryption} to encrypt the model, which allows other nodes to use the model without decrypting it.

Future versions of DFL will integrate these solutions to prevent these types of attacks. %since it is still at the prototype level.  

% Model duplication attack is a new attack method which only exists in blockchain federated machine learning system. The threat model can be described as the attacker duplicates the model from other innocent nodes, and generate a new transaction with the duplicated model to gain contributions to the model. Verifying the digest of transaction does not solve it because the attacker can slight modify the model weights to get a completely different digest and retain similar accuracy. 

% There are two mainstream solutions to this attack, one is use Trusted Execution Environments (TEEs) on all nodes to protect the model data, another way is using homomorphic encryption to encrypt the model and allow other nodes to use it without decrypting it.

% However, DFL integrates neither of above solutions since it is still at the prototype level. 
